Federated Multi-Sequence Stochastic Approximation with Local Hypergradient Estimation

Stochastic approximation with multiple coupled sequences (MSA) has found broad applications in machine learning as it encompasses a rich class of problems including bilevel optimization (BLO), multi-level compositional optimization (MCO), and reinforcement learning (specifically, actor-critic methods). However, designing provably-efficient federated algorithms for MSA has been an elusive question even for the special case of double sequence approximation (DSA). Towards this goal, we develop FedMSA which is the first federated algorithm for MSA, and establish its near-optimal communication complexity. As core novelties, (i) FedMSA enables the provable estimation of hypergradients in BLO and MCO via local client updates, which has been a notable bottleneck in prior theory, and (ii) our convergence guarantees are sensitive to the heterogeneity-level of the problem. We also incorporate momentum and variance reduction techniques to achieve further acceleration leading to near-optimal rates. Finally, we provide experiments that support our theory and demonstrate the empirical benefits of FedMSA. As an example, FedMSA enables order-of-magnitude savings in communication rounds compared to prior federated BLO schemes.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}
% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}



% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\lpa{{\left(}}
\def\rpa{{\right)}}
\def\lcb{{\left\{}}
\def\rcb{{\right\}}}
\def\lbr{{\left[}}
\def\rbr{{\right]}}
\def\lnr{{\left\|}}
\def\rnr{{\right\|}}
\def\lan{{\left\langle}}
\def\ran{{\right\rangle}}

\def\norm[1]{\lnr#1\rnr}
\def\normb[1]{\big\|#1\big\|}

\def\nn{{\nonumber}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\summM{{\sum_{m=1}^M}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/actor_critic.tex <==
% \section{Application to Federated Actor-Critic}

% We will follow the exposition of the prior convergence results on actor-critic methods \cite{chen2021closing,hong2020two}.





==> sec/app_related.tex <==

\begin{lemma}[Counterpart of Lemma~\ref{thm4:lemma2}]\label{thm4:s:lemma2}
Suppose Assumptions~\ref{assu:s:f} and \ref{assu:s:bound:var} hold. Further, assume $\tau_i \geq 1$ and $\alpha_i=\alpha/\tau_i, \forall i \in \mathcal{S}$, where $\alpha \leq 1/(3 L_f)$. Then, for all $\nu \in \{0,\ldots, \tau_i-1\}$, \fedout gives
\begin{align}\label{eqn1:lemm:s:drift}
 \mb{E}\left[\left\|\m{x}_{i,\nu}-\m{x}\right\|^2\right]\leq 12 \tau_i^2 \alpha_i^2  \mathbb{E}\left[\left\|\nabla  f(\m{x})\right\|^2\right] +  27 \tau_i \alpha_i^2 \sigma_f^2.
\end{align}
\end{lemma}
\begin{proof}
The result trivially holds for $\tau_i=1$. Similar to what is done in
the proof of Lemma~\ref{thm4:lemma2}, let $\tau_i>1$ and define
\begin{equation}\label{eqn1+:s:lemm:drift}
\begin{aligned}
\m{v}_{i,\nu}&:=\nabla f_i(\m{x}_{i,\nu})- \nabla f_i(\m{x}) + \nabla f (\m{x}),\\
\m{w}_{i,\nu}&:= \m{h}_i(\m{x}_{i,\nu})-\nabla f_i(\m{x}_{i,\nu})+  \nabla f_i(\m{x})-\m{h}_i(\m{x})+\m{h}(\m{x})- \nabla f(\m{x}).
\end{aligned}
\end{equation}
%where  $ \m{h}(\m{x})=
%1/m\sum_{i=1}^m \nabla_{\m{x}} f_i(\m{x};\xi_{i})$, $\m{h}_i(\m{x})=\nabla_{\m{x}} f_i(\m{x};\xi_{i,\nu})$, and $ \m{h}_i(\m{x}_{i,\nu})=\nabla_{\m{x}} f_i(\m{x}_{i,\nu};\xi_{i,\nu})- \m{h}_i(\m{x}) + \m{h}(\m{x})$.  

From Algorithm~\ref{alg:fedout}, for each $i\in\mathcal{S}$, and $\forall  \nu \in\{0,\ldots,\tau_i-1\}$, we obtain
\begin{equation*}
\begin{aligned}
        \m{x}_{i,\nu+1}-\m{x}&=\m{x}_{i,\nu}-\m{x}-\alpha_i \left(\m{h}_i(\m{x}_{i,\nu})-\m{h}_i(\m{x})+\m{h}(\m{x})\right)\\
        %  &= \m{x}_{i,\nu}-\m{x}-\alpha_i \left(\m{v}_{i,\nu}+\m{w}_{i,\nu}\right),
    \end{aligned}
\end{equation*}
which implies that 
% Now, iterating equation \eqref{eqn4:s:lemm:drift} and using $\m{x}_{i,0}=\m{x}, \forall i\in\mathcal{S}$, we obtain
\begin{equation}
\label{eqn6:lemm:drift}
    \begin{aligned}
        \mb{E}\left[\|\m{x}_{i,\nu}-\m{x}\|^2\right]&\leq  \left(   4 \tau_i \alpha_i^2  \mb{E}\left[\|\nabla f(\m{x})\|^2\right] +9 \alpha_i^2\sigma_f^2 \right) \sum\limits_{j=0}^{\nu -1} \left(1+\frac{1}{\tau_i-1}\right)^j\\
        &\leq 12 \tau_i^2 \alpha_i^2  \mb{E}\left[\|\nabla f(\m{x})\|^2\right] +27\tau_i \alpha_i^2 \sigma_f^2,
    \end{aligned}
\end{equation}
where the second inequality uses \eqref{eqn:sum:geom}. This completes the proof.

\begin{equation}\label{eqn2:s:lemm:drift}
\begin{aligned}
\mb{E}\left[\|\m{x}_{i,\nu+1}-\m{x}\|^2\right]
&=\mb{E}\left[\|\m{x}_{i,\nu}-\m{x}-\alpha_i \m{v}_{i,\nu}\|^2\right]+\alpha_i^2\mb{E}\left[\|{\m{w}_{i,\nu}}\|^2\right]\\&-2\mb{E}\left[\mb{E}\left[\langle \m{x}_{i,\nu}-\m{x}-\alpha_i\m{v}_{i,\nu},\alpha_i \m{w}_{i,\nu} \rangle\mid\mathcal{F}_{i,\nu-1}\right]\right] \\ 
&= \mb{E}\left[\|\m{x}_{i,\nu}-\m{x}-\alpha_i\m{v}_{i,\nu}\|^2\right]+\alpha_i^2\mb{E}\left[\|\m{w}_{i,\nu}\|^2\right].
\end{aligned}
\end{equation}
Here, the last equality uses Lemma~\ref{lem:rand:zer} since  $\mb{E}[\m{w}_{i,\nu}|\mathcal{F}_{i,\nu-1}]=0$.


From  Assumption~\ref{assu:s:bound:var} and Lemma~\ref{lem:Jens}, for $\m{w}_{i,\nu}$ defined in \eqref{eqn1+:s:lemm:drift}, we have
\begin{equation}
\label{eqn3b:s:lemm:drift}
\begin{aligned}
\mb{E}\left[\|\m{w}_{i,\nu}\|^2\right] &\leq 3   \mb{E}\left[\|\m{h}_i(\m{x}_{i,\nu})-\nabla f_i(\m{x}_{i,\nu})\|^2+\|\nabla f_i(\m{x})-\m{h}_i(\m{x})\|^2+\|\m{h}(\m{x})- \nabla  f  (\m{x})\|^2\right]\\
        & \leq 9\sigma_f^2.
    \end{aligned}
\end{equation}
Substituting  \eqref{eqn3b:s:lemm:drift} into \eqref{eqn2:s:lemm:drift}, we get
\begin{equation}
\label{eqn4:s:lemm:drift}
\begin{aligned}
\mb{E}\left[\|\m{x}_{i,\nu}-\m{x}-\alpha_i\m{v}_{i,\nu}\|^2\right] &\leq  \left(1+\frac{1}{2\tau_i-1}\right)\mb{E}\left[\|\m{x}_{i,\nu}-\m{x}\|^2\right]+ 2\tau_i \alpha_i^2 \mb{E}\left[\|\m{v}_{i,\nu}\|^2\right] +9 \alpha_i^2\sigma_f^2 \\
       &\leq  \left(1+\frac{1}{2\tau_i-1}+4 \tau_i \alpha_i^2 L_f^2\right)\mb{E}\left[\|\m{x}_{i,\nu}-\m{x}\|^2\right]
 + 4 \tau_i \alpha_i^2  \mb{E}\left[\|\nabla f(\m{x})\|^2\right] +9 \alpha_i^2\sigma_f^2\\
        &\leq  \left(1+\frac{1}{\tau_i-1}\right)\mb{E}\left[\|\m{x}_{i,\nu}-\m{x}\|^2\right]+ 4 \tau_i \alpha_i^2  \mb{E}\left[\|\nabla f(\m{x})\|^2\right] +9 \alpha_i^2\sigma_f^2.
    \end{aligned}
\end{equation}
Here, the first inequality follows from Lemma~\ref{lem:trig}; the second inequality uses Assumption~\ref{assu:s:f} and Lemma~\ref{lem:Jens};
and the last inequality follows by noting $\alpha_i=\alpha/\tau_i, \forall i \in \mathcal{S}$ and $\alpha \leq 1/(3 L_f)$.
\end{proof}


\subsection{Federated Estimator~II (Douglas-Rachford Splitting)} 
Douglas-Rachford (DR) splitting is an efficient first-order method which models the optimization problem as the problem of finding a zero of the sum of monotone operators. 
\begin{wrapfigure}{r}{0.5\textwidth}
\begin{minipage}{0.5\textwidth}
\vspace{-8mm}
\begin{algorithm}[H]
    \centering
    \caption{Example Algorithm}\label{algo:FDR}
    \begin{algorithmic}[1]
  \caption{$\m{s}^+=~\pmb{\mc{B}}~(\m{b},\m{s},\eta)$
  }
  %\For {$n=0,\ldots,N-1$} 
  %\State Compute an unbiased estimator $\hat{\m{b}}_i$ of $\m{b}_i$
   \State $\m{v}_{i0} =\m{b}_i+ 2\m{s}-\m{z}_{i}$
  \For{$\nu=0,\ldots, \tau_i-1$}
  %	\State Compute an unbiased estimator $\hat{\m{A}}_i$ of $\m{A}_i$
        \State $\m{v}_{i,\nu+1}= \eta \m{v}_{i}+\left(\m{I}-\eta \m{A}_i(\xi_{i,\nu})\right) \m{v}_{i,\nu}$
        \EndFor
%         \State $\m{y}_{i,k}= \m{p}_{i,n}$
                \State $\m{z}_{i}^{+} = \m{z}_{i} + \m{v}_{i,\tau_i}-\m{s}$   
    %    \EndFor
        \State $\m{s}^+ = m^{-1}\sum_{i\in\Sc}\m{z}_{i}$
        %\EndFor
     %   \EndFor
    \end{algorithmic}
\end{algorithm}
 \end{minipage}
 \end{wrapfigure}
In order to use DR for federated second-order optimization, we first transform problem \eqref{eqn:lsys:main} into the {\em consensus form}
\begin{equation}\label{obj:consensus:form}
 \min_{\m{z} \in \mb{R}^{mp}} \sum_{i=1}^m\phi_i^1(\m{z}_i) + \phi^2(\m{z}).
\end{equation}
Here, $\phi_i^1(\m{z})=\|\m{A}_i \m{z}_i - \m{b}_i\|^2$, $\m{z}_1,\dots, \m{z}_m \in \mb{R}^p$ are independent copies of $\m{z}$, $\phi^2:\mb{R}^{mp}\to \mb{R}$ is a regularizer given by
\begin{equation}\label{eq:constraint:consensus}
\phi^2(\m{z}):= 
	\begin{cases}
		0, & \textrm{if } \m{z}_1=\ldots=\m{z}_n\,, \\
		+\infty, & \textrm{otherwise},
	\end{cases}
\end{equation}
corresponding to the following consensus constraint $\mc{C}:= \left\{(\m{z}_1,\dots,\m{z}_n) \in \mb{R}^{mp}~:\m{z}_1=\ldots=\m{z}_m\right\}.$ Given a proper, closed and convex function $h:\mb{R}^d \to \mb{R} \cup \{+\infty\}$ and $\gamma > 0$, the proximal operator $\text{prox}_{\gamma h}:\mb{R}^p \to \mb{R}^p$ is defined as
\begin{align}
\prox_{\gamma h}(\m{x}) = \text{argmin}_\m{y} \left\{h(\m{y}) + \frac{1}{2\gamma}\|\m{x} - \m{y}\|_2^2\right\}.
\end{align}
In the case $h = \phi^2$, evaluating the proximity operator of \eqref{eq:constraint:consensus} amounts to taking the average of the variables: $\text{prox}_{\phi^2}(\m{z}_1,\dots,\m{z}_m)= (\bar{\m{z}},\dots,\bar{\m{z}})\in \mb{R}^{mp},$
where $\bar{\m{z}} = \frac{1}{m}\sum_{i=1}^m \m{z}_i$. Starting from some \(\m{z}\in\mb{R}^p\), one iteration of DRS applied to \eqref{eq:constraint:consensus} amounts to
		\[
			\tag{DRS}\label{DRS}
			\begin{cases}%[lcl]
\m{z}_{i}^{k+\frac{1}{2}} =\prox_{\phi_i^1}(2\m{s}^k-\m{z}_{i}^k)\\%=
\m{z}_{i}^{k+1} = \m{z}_{i}^k +   \m{z}_{i}^{k+\frac{1}{2}} -\m{s}^k\\
\m{s}^{k+1} =\prox_{\phi^2}(\m{z}_{i}^{k+1})  
\end{cases}
		\]
We now describe a method, derived from splitting the inclusion relation, whose fixed points do correspond with global minima of \eqref{obj:consensus:form} \red{Is this for ridge regularization with $\gamma=1$ or for unregularized $\gamma=\infty$?}. It is an instantiation of the Douglas-Rachford splitting, which we refer to as the \feddr algorithm in this distributed setting. The derivation is in Appendix
% \hfill
%
\begin{theorem}\label{thm:DR+Neumann:convergence}
For any initialization $\m{z}^{(1)} \in \mb{R}^d$, Algorithm~\ref{algo:FDR} with stepsize $\eta = O(1/\sqrt{\ell_{f,1} \mu})$
satisfies
\begin{align}%\label{eqn:fedDR:bound}
\nonumber 
\mb{E}\left[\|\m{s}^{(t+1)} - \m{s}^\star\|\right] &\leq \left(1 - \frac{2}{\sqrt{\kappa} +
  1}\right)^{\! t}\frac{\|\m{s}^{(1)} -\m{s}^\star\|}{\sqrt{m}} + \mc{E}_{\textnormal{Neumann}}. 
\end{align}
Here, $\mc{E}_{\textnormal{Neumann}}$ is the Neumanm approximation error which can be bounded as  
%  & + (\sqrt{\kappa} + 1) \left(\frac{1}{\mu} \left(\frac{\kappa-1}{\kappa} \right)^N + N {\eta}^2 \sigma^2_{g,2}\right).
\end{theorem}

Theorem~\ref{thm:DR+Neumann:convergence}   



\section{Extended Related Work}\label{supp:sec:related}

Here we discuss additional references that were omitted from Section \ref{sec related} due to limited space.



==> sec/fedbilevel.tex <==
\section{Applications to Newton's Method and Bilevel Optimization}\label{sec:application}
\subsection{Federated Newton Method} 
\begin{wrapfigure}{r}{0.5\textwidth}
\begin{minipage}{0.5\textwidth}
\vspace{-8mm}
\begin{algorithm}[H]
\caption{\pmb{\textnormal{FedNewton}}}
\label{alg:fedblo}
\begin{algorithmic}[1]
\State \textbf{Inputs:} $K,N \in \mb{N}$;~~$(\m{x}^0,\m{s}^0)\in \mb{R}^{2d_1}$;~~\textbf{\pmb{\mc{A}}},\\
\hspace{33pt}\pmb{\mc{B}} with stepsizes $\{\eta^k, \alpha^k\}_{k=0}^{K-1}$
%	    \While{not converged}
\For{$k = 0, \cdots, K-1$}
		\State \textbf{Option~A:} $\m{s}^k=~\pmb{\mc{A}}~(\m{s}^{k-1}, \eta, N)$
		\State \textbf{Option~B:} $\m{s}^k=~\pmb{\mc{B}}~(\m{s}^{k-1}, \eta, N)$
				\State $\m{x}^{k+1}=\m{x}^{k}-\alpha^k \m{s}^k$
		\EndFor	

\end{algorithmic}
\end{algorithm}
 \end{minipage}
 \end{wrapfigure}
The canonical example of second-order methods to solve  \eqref{fedsingle:prob} is arguably the classical Newton’s method whose iterations are typically written as 
\begin{equation*}
    \m{x}^{k+1} = \m{x}^{k} - \alpha^k\mathbf{H}_k^{-1}\mathbf{g}_k,
\end{equation*}
where $k$ denotes the $k$-th iteration, $\m{g}_k = \mathbf{g}(\m{x}^k) = \nabla f (\m{x}^k)$ is the gradient at iteration $k$ and $\eta_k$ is the step size (also called learning rate) at iteration $k$. $\m{H}_k = \nabla^2 f (\m{x}^k)$ denotes the Hessian matrix at iteration $k$. Compared to gradient descent, the Newton method exploits the curvature information provided by the Hessian matrix to improve the descent direction. We define $\m{s}^k := \m{H}_k^{-1}\m{g}_k$.
We make the following assumptions on inner/outer objectives. 
\vspace{0.1cm}
% \noindent\textbf{Assumption 1 (Lipschitz continuity).}
%
\begin{assumption}[Well-behaved objectives]\label{assu:s:f} 
%\noindent   {\bf Assumptions A}
For all $i \in [m]$:
\begin{enumerate}[label={\textnormal{\textbf{(A\arabic*})}}]
%[label={\textbf{(a\arabic*})}]
\vspace{-.3cm}
\item %[\textbf{a)}]
$\nabla f_i(\m{z}), \nabla^2 f_i (\m{z})$ are $\ell_{f,1}$, $\ell_{g,2}$-Lipschitz continuous, respectively%; and 
\vspace{-.2cm}
% \item % [\textbf{d)}]
% $g_i(\m{x},\m{y})$ is $\mu_{g}$-strongly convex in $\m{y}$ for all $\m{x}\in \mb{R}^{d_1}$.
\end{enumerate}
\end{assumption}
Throughout, we use $\kappa_f=\ell_{f,1}/\mu_f$ to denote the condition number of the inner function $f$.
\begin{assumption}[Stochastic samples]\label{assu:s:bound:var}
For all $i \in [m]$:
\begin{enumerate}[label={\textnormal{\textbf{(B\arabic*})}}]
\vspace{-.3cm}
\item $\nabla f_i(\m{z};\xi)$, $\nabla^2 f_i(\m{z}; \xi)$ are unbiased estimators of $\nabla f_i(\m{z})$,  $\nabla^2f_i(\m{z})$, respectively; and
%$\mb{E}_{\xi}[\nabla f_i(\m{z};\xi)]=\nabla f_i(\m{z})$, $\mb{E}_{\zeta}[\nabla g_i(\m{z};\zeta)]=\nabla g_i(\m{z})$, $\mb{E}_{\zeta}[\nabla^2 g_i(\m{z}, \zeta)=\nabla g_i(\m{z})]$
%are unbiased estimators of $\nabla f_i(\m{z})$, $\nabla g_i(\m{z})$, and $\nabla^2g_i(\m{z})$, respectively;
\item Their variances are bounded, i.e., $\mb{E}_{\xi}[\|\nabla f_i(\m{z};\xi)-\nabla f_i(\m{z})\|^2] \leq \sigma_{f,1}^2$,  and $\mb{E}_{\zeta}[\|\nabla^2 f_i(\m{z};\zeta)-\nabla^2 f_i(\m{z})\|^2] \leq \sigma_{f,2}^2$ for some $\sigma_{f,1}^2$, and $\sigma_{f,2}^2$.
\end{enumerate}
\end{assumption}

\begin{theorem}[\textbf{Linear-Quadartic Rate}]\label{thm:fednewton}
Suppose Assumptions~\ref{assu:s:f} and \ref{assu:s:bound:var} hold.  %Further, assume $\alpha_i^k=\alpha_k/\tau_i$ for all $ i \in \mathcal{S}$, where
Then, 
	\begin{equation}  \label{capsule}
	\E \left[\|\m{x}^{k+1}-\m{x}^*\|\right] \leq C_1 \|\m{x}^k -\m{x}^*\|^2+\left( \frac{C_2}{\sqrt{\beta}} +C_3 \theta^r \right) \|\m{x}^k-\m{x}^*\| + C_4,
	\end{equation}
	where    
	\begin{equation}   \label{c3}
	C_1=, \quad C_2 =, \quad   
	C_3 = , C_4= \quad \theta=, \quad
	\delta(\beta)= .
	\end{equation}
%  \begin{align}\label{eqn:param:s:choice}
%  \alpha_k&=\min\left\{\bar{\alpha}_1,\frac{\bar{\alpha}}{\sqrt{K}}\right\}
%  \end{align}
%  for some positive $\bar{\alpha}_1$ and  $\bar{\alpha}$. Then,

 
 
% \begin{enumerate}[label=\textnormal{(\Roman*)}]
% \item \label{itm:thm:fednew:a} If ...
% \item \label{itm:thm:fednew:b} If 
% \begin{equation*}
%  \frac{1}{K} \sum_{k=1}^K\mb{E}\left[\left\|\nabla f(\m{x}^k)\right\|^2\right]=\mc{O}\left( \frac{ \Delta_f}{ \bar{\alpha}_1 K} + \frac{  \frac{\Delta_f}{\bar{\alpha}} + \bar{\alpha}\sigma_f^2 }{\sqrt{K}}\right),
% \end{equation*}
% where $\Delta_{f}:= f(\m{x}^0)-\mb{E}[f(\m{x}^K)]$.
% \end{enumerate}
 \end{theorem}

\subsection{Federated Bilevel Optimization}

==> sec/fedihgp.tex <==
    
    \begin{algorithm}[t]
  \caption{$\m{p}_{N'}=~\pmb{\fedhess}~(\m{x}, \m{y}^+,N)$: Federated approximation of inverse-Hessian-gradient product}
\begin{algorithmic}[1]
%\For{$t=T-1,...,0$}
\State Select $ N'\in \{0, \dots, N-1\}$ UAR.
\State Select $\mc{S}_0 \in \mc{S}$ UAR.
%\State If $N'=0$ 
  \For{$i \in \mc{S}_0$ \textbf{in parallel}} 
 \State $\m{p}_{i,0} =\nabla_\m{y} f_i(\m{x}, \m{y}^+; \xi_{i,0})$
 \EndFor
 \State $ \m{p}_0 = \frac{N}{\ell_{g,1}}  |\mc{S}_0|^{-1}\sum_{i\in\mathcal{S}_0} \m{p}_{i,0}$  %\hspace{.5cm}\texttt{\#communication}  
\If{$N'=0$}
\State  Return $\m{p}_{N'}$
\EndIf
%  \State{{\color{blue} Option~I (Local Inverse):} 
%  \State Select $\mc{S}_{ N'} \in \mc{S}$ UAR.}
%   		\For {$i \in \mc{S}_{N'}$ \textbf{in parallel}} 
% 		 \State $\m{p}_{i,N'} = \prod\limits_{n=1}^{N'} \big(\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_y g_i(\m{x}, \m{y}^+;{\zeta}_{i,n})\big)\m{p}_{0}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y}^+;\xi_j)$}
% 	   \EndFor
% 	   \State $\m{p}_{N'}= |\mc{S}_{N'}|^{-1}\sum_{i\in\mc{S}_{N'}} \m{p}_{i,N'}$ 
%\State{{\color{blue} Option~II (Global Inverse):}}
\State Select $\mc{S}_1, \ldots, \mc{S}_{ N'} \in \mc{S}$ UAR.
\For{$n=1,\ldots, N'$}
 	   % \State Choose $N' \in \{0,\ldots,N-1\}$ randomly and 
	%	\For {$i \in \mc{S}$ \textbf{in parallel}} 
		\For {$i \in \mc{S}_n$ \textbf{in parallel}} 
		 \State $\m{p}_{i,n} = \left(\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_\m{y} g_i(\m{x}, \m{y}^+;{\zeta}_{i,n})\right)\m{p}_{n-1}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y}^+;\xi_j)$}
	   \EndFor
	   \State $\m{p}_{n}=|\mc{S}_n|^{-1}\sum_{i\in\mc{S}_n} \m{p}_{i,n}$ %\hspace{.5cm}\texttt{\#communication}  
	   %\Else 
 	   %\State $\m{p}_{i}^{k,t}=\m{p}^{k,t+1}-\beta_i \nabla_\m{y}^+^2  g_i (\m{x},\m{y}^+)\m{p}^{k,t+1}$~~ 
	   %\EndFor
	%	\State $\m{p}^{k,t}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i}^t$
	%	\State { $\m{p}^k=\sum_{t=0}^{T-1}\m{p}^{k,t}$}
		\EndFor
%\State  Set $\m{p}_{N}= \frac{N}{\ell_{g,1}} \m{p}_{N'}$. Return $\m{p}_N$		
\end{algorithmic}\label{fedihgp_algo}
\end{algorithm}

%\ct{Should $\mathbf{p}_0$ change to use local iterates $x_{i,\ell}$ for OPTION 1? At least, to agree with $h_{i}(x_{i,\ell},y)$.}

==> sec/fedinn.tex <==
\begin{algorithm}[t]
\caption{$ \m{y}^+~=~\pmb{\fedinn}~(\m{x},\m{y},\beta$) 
%for stochastic \colorbox{cyan!30}{bilevel (\func$\gets$)}, \colorbox{green!30}{minimax (\func$\gets$)}, and \colorbox{magenta!30}{compositional (\func$\gets$)} problems
}
\label{alg:fedinn}
\begin{algorithmic}[1]
%\For{$t\in(T]$} 
%Set query function 
\State $\funcin_i(\cdot)\gets$ \colorbox{cyan!30}{$\nabla_\m{y} g_i(\m{x},\cdot)$~\text{(bilevel)}},\colorbox{green!30}{$-\nabla_\m{y} f_i(\m{x},\cdot)$~\text{(minimax)}}
%\colorbox{magenta!30}{$-h_i(\cdot)$~\text{(composite)}},\\
%\hspace{37pt}
%\funcin_i\gets 
 \State $\m{y}_{i,0}=\m{y}$ and $\beta_i \in (0,\beta]$
  \For{$i \in \mc{S}$ \textbf{in parallel}} 
 \State $\m{q}_i=\funcin_i(\m{y};  \zeta_{i})$
%\State \colorbox{green!30}{$\m{q}_i=-\nabla_\m{y} f_i(\m{x}, \m{y};  \xi_{i})$}
% \State \colorbox{magenta!30}{$\m{q}_i=-h_i(\m{x}; \zeta_{i})$}
 \EndFor
 \State $\m{q}=|\mathcal{S}|^{-1}\sum_{i\in\mathcal{S}}\m{q}_i$ %\hspace{1.5cm}\texttt{\#communication}  
 \For {$i \in \mc{S}$ \textbf{in parallel}} 
 %\State Choose $\beta_i \in (0, \beta)$
\For {$\nu=0,\ldots,\tau_i-1$} 
%\vspace{2mm}
\State $\m{q}_{i,\nu }=\funcin_i(\m{y}_{i,\nu };\zeta_{i,\nu })-\funcin_i(\m{y};\zeta_{i,\nu })+\m{q}$
%\State \colorbox{green!30}{$ \m{q}_{i,\nu }=-\nabla_\m{y} f_i(\m{x}, \m{y}_{i,\nu };\xi_{i,\nu })+\nabla_\m{y} f_i(\m{x}, \m{y};\xi_{i,\nu })$}
%\State \colorbox{magenta!30}{$ \m{q}_{i,\nu }=h_i(\m{x}_{i,\nu };\zeta_{i,\nu })-h_i(\m{x};\zeta_{i,\nu })$}
\State $\m{y}_{i,\nu +1}= \m{y}_{i,\nu }-\beta_i\m{q}_{i,\nu }$
\EndFor
\EndFor
\State $\m{y}^{+}=|\mathcal{S}|^{-1}\sum_{i\in\mathcal{S}}\m{y}_{i,\tau_i}$ %\hspace{1cm}\texttt{\#communication}  
%\EndFor
\end{algorithmic}
\end{algorithm}
% \begin{algorithm}[t]
% \caption{$ \m{y}^T ~=~\pmb{\fedinn}~(\m{x},\m{y}^{0},T,\beta$) for stochastic \colorbox{red!30}{bilevel} and \colorbox{green!30}{minimax} problems}
% \label{algo:svrg}
% \begin{algorithmic}[1]
% %\For{$t\in(T]$} 
%   \For{$i \in \mc{S}$ \textbf{in parallel}} 
%  \State \colorbox{red!30}{$\m{q}^t_i=\nabla_y g_i(\m{x}, \m{y}^{t};  \zeta_{i}^t)$}
%  \State \colorbox{green!30}{$\m{q}^t_i=-\nabla_y f_i(\m{x}, \m{y}^{t};  \xi_{i}^t)$}
%  \EndFor
%  \State $\m{q}^t=|\mathcal{S}|^{-1}\sum_{i\in\mathcal{S}}\m{q}^t_i$
%  \State $\m{y}^t_{i,0}=\m{y}^t$
%  \For {$i \in \mc{S}$ \textbf{in parallel}} 
%  %\State Choose $\beta_i \in (0, \beta)$
% \For {$\ell=0,\ldots,\tau_i-1$} 
% %\vspace{2mm}
% \State \colorbox{red!30}{$\m{q}_{i,\nu }^t=\nabla_y g_i(\m{x}, \m{y}^t_{i,\nu };\zeta_{i,\nu }^t)-\nabla_y g_i(\m{x}, \m{y}^{t};\zeta_{i,\nu }^t)$}
% \State \colorbox{green!30}{$ \m{q}_{i,\nu }^t=-\nabla_y f_i(\m{x}, \m{y}^t_{i,\nu };\xi_{i,\nu }^t)+\nabla_y f_i(\m{x}, \m{y}^{t};\xi_{i,\nu }^t)$}
% \State $\m{y}^{t}_{i,\nu +1} \gets \m{y}^{t}_{i,\nu }-\beta_i (\m{q}_{i,\nu }^t+\m{q}^t)$
% \EndFor
% \EndFor
% \State $\m{y}^{t+1}=|\mathcal{S}|^{-1}\sum_{i\in\mathcal{S}}\m{y}^t_{i,\tau_i}$
% %\EndFor
% \end{algorithmic}
% \end{algorithm}

==> sec/fedout.tex <==
\begin{algorithm}[t]
\caption{$\m{x}^{+} ~=~\pmb{\fedout}~(\m{x}, \m{y}^+, \alpha)$ for stochastic \colorbox{cyan!30}{bilevel} and  \colorbox{green!30}{minimax} problems
%
%\ct{Maybe change input to $\y^{+}$ for consistency with section?}
%,
%and \colorbox{magenta!30}{compositional} 
} %\colorbox{purple!30}{SVRG}}
\begin{algorithmic}[1]
\State $\funco_i(\cdot)\gets \nabla_\m{x} f_i(\cdot,\m{y}^+;\cdot)$ %(bilevel \& min-max), 
%\\
%\hspace{30pt}\colorbox{magenta!30}{$\gets \nabla_\m{x} h_i(.) \nabla_\m{y}^+ f_i(.)$~(compositional)}   
%\colorbox{cyan!30}{$\nabla_\m{y}^+ f_i(\cdot)$~\text{(bilevel)}}, \colorbox{green!30}{$-\nabla_\m{y}^+ f_i(\cdot)$~\text{(min-max)}},\\ \hspace{35pt}\colorbox{magenta!30}{$-h_i(\cdot)$~\text{(composite)}}%\func_i\gets 
 \State $\m{x}_{i,0}=\m{x}$ and $\alpha_i \in (0,\alpha]$
\State \colorbox{cyan!30}{Choose $N \in \mb{N}$ and set $ \m{p}_{N^{'}}=~\pmb{\fedhess}~(\m{x}, \m{y}^+,N)$}
 \For{$i \in \mc{S}$ \textbf{in parallel}} 
 \State \colorbox{cyan!30}{$\m{h}_i= \funco_i(\m{x};\xi_{i})-\nabla^2_{\m{xy}}g_i(\m{x},\m{y}^+;{\zeta}_{i})
 \m{p}_{N^{'}}$}
% \State \colorbox{green!30}{$\m{h}_i=\funco_i(\m{x};  \xi_{i})$},  \colorbox{magenta!30}{$\m{h}_i= \nabla h_i(\m{x};  \zeta_{i}) \nabla f_i(\m{y}^+;  \xi_{i})$}
  \State \colorbox{green!30}{$\m{h}_i=\funco_i(\m{x};  \xi_{i})$}
 %  \State   \colorbox{magenta!30}{$\m{h}_i= \nabla^2_{\m{xy}}g_i(\m{x},\m{y}^+;{\zeta}_{i})
 %\m{p}_0$}
 \EndFor
 \State $\m{h}=|\mathcal{S}|^{-1}\sum_{i\in\mathcal{S}}\m{h}_i$ %\hspace{1.5cm}\texttt{\#communication}    
 \For {$i \in \mc{S}$ \textbf{in parallel}} 
\For {$\nu= 0,\ldots,\tau_i-1$} 
 %\State Choose $\beta_i \in (0, \beta)$
% \For {$i \in \mc{S}$ \textbf{in parallel}} 
 \State%\colorbox{cyan!30}{
$\m{h}_{i,\nu }=\funco_i(\m{x}_{i,\nu }; \xi_{i,\nu })-\funco_i(\m{x}; \xi_{i,\nu })+\m{h}$
%\colorbox{magenta!30}{$\m{h}_{i,\nu }= \nabla h_i(\m{x}_{i,\nu };  \zeta_{i}) \nabla f_i(\m{y}^+_{i,\nu };  \xi_{i,\nu })+ \nabla h_i(\m{x};  \zeta_{i}) \nabla f_i(\m{y}^+_{i,\nu };  \xi_{i,\nu })$
%}
 %}%\colorbox{purple!30}{SVRG}
% \State \colorbox{red!30}{$ \m{h}_{i,\nu }= \nabla_{\m{x}} f_i(\m{x}, \m{y}^+^*(\m{x}))-\nabla^2_{\m{xy}}g_i(\m{x},\m{y}^+^*(\m{x}))
% \m{p}_N $}-%\colorbox{purple!30}{SVRG}
% \State\colorbox{green!30}{$\m{h}_{i,\nu }=\nabla_{\m{x}} f_i(\m{x}_{i,\nu }, \m{y}^+; \xi_{i,\nu })-\nabla_{\m{x}} f_i(\m{x}, \m{y}^+; \xi_{i,\nu })$}%\colorbox{purple!30}{SVRG}
%\State \colorbox{magenta!30}{$\m{h}_{i,\nu }=-\nabla_y f_i(\m{x}, \m{y}^+;  \xi_{i})$}
 %\State \colorbox{magenta!30}{$\m{h}_i=\nabla h_i(\m{x}_{i,\nu };  \zeta_{i,\nu }) \nabla f_i(\m{y}^+_{i,\nu };  \xi_{i,\nu })-\nabla h_i(\m{x}; \zeta_{i,\nu }) \nabla f_i(\m{y}^+;  \xi_{i,\nu })$}
 %~~\Comment{via automatic differentiation}
% \State  $\m{H}_i^{k+1} = \m{H}_i^k + \pi_1 \m{S}_i^k$ and $\m{J}_i^{k+1} = \m{J}_i^k + \pi_2\m{W}_i^k$;
% %\Stae Send $\nabla f_i(x^k)$,\; $\mS_i^k \eqdef \cC_i^k(\nabla^2 f_i(x^k) - \mH_i^k)$ and $l_i^k \eqdef \|\mH_i^k - \nabla^2 f_i(x^k)\|_{\rm F}$ to the server
%\State  $\m{x}^{+}=1/m\sum_{i\in\mathcal{S}}\m{x}_{i}$
 \State  $ \m{x}_{i,\nu +1}= \m{x}_{i,\nu }- \alpha_i\m{h}_{i,\nu }$%~~\Comment{via automatic
  \EndFor
\EndFor
\State $\m{x}^{+}=|\mc{S}|^{-1}\sum_{i\in \mc{S}} \m{x}_{i,\tau_i}$ %\hspace{1cm}\texttt{\#communication}  
% \EndFor
\end{algorithmic}
\label{alg:fedout}
\end{algorithm}







% Estimator~\eqref{eq.inverse-estimator} is not time and memory efficient to compute in  federated setting due to the summation inverse in \eqref{eqn:grad:y}. Besides, in 

%It can be easily seen that the above procedure gives an estimate of $\tilde{\nabla}f(\m{x},\m{y})$ with three rounds of vector communication with the server.


% \begin{figure*}
%  \begin{subfigure}{.47\textwidth}

%  \end{subfigure}
%   \hspace*{0.03in}
%  \begin{subfigure}{.5\textwidth}
%   \tiny{
% \begin{algorithm}[H]
%   \caption*{$\m{x}^{+} ~=~\pmb{\fedout}~(\m{x}, \m{y}, \alpha,N$ }
% \begin{algorithmic}[1]
% %\For{$t=T-1,...,0$}
% \State Select $ N'\in \{1, \dots, N\}$ and $\mc{S}_0, \ldots, \mc{S}_{ N'+1} \in \mc{S}$ uniformly at random.
%   \For{$i \in \mc{S}_0$ \textbf{in parallel}} 
%  \State Compute $\nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$
%  \EndFor
%  \State $ \m{p}_0 \leftarrow 1/|\mc{S}_0|\sum_{i\in\mathcal{S}_0} \nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$ 
%  	%	\State $\m{p}_{i,0}\leftarrow \m{p}$
%  		 \For{$n=1,\ldots, N'$}
%  	   % \State Choose $N' \in \{0,\ldots,N-1\}$ randomly and 
% 	%	\For {$i \in \mc{S}$ \textbf{in parallel}} 
% 		\For {$i \in \mc{S}_n$ \textbf{in parallel}} 
% 		 \State $\m{p}_{i,n} \leftarrow (\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_y g_i(\m{x}, \m{y};{\zeta}_{i,n}))\m{p}_{n-1}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y};\xi_j)$}
% 	   \EndFor
% 	   \State $\m{p}_{n}\leftarrow 1/|\mc{S}_n|\sum_{i\in|\mc{S}_n|} \m{p}_{i,n}$
% 	   %\Else 
%  	   %\State $\m{p}_{i}^{k,t}=\m{p}^{k,t+1}-\beta_i \nabla_\m{y}^2  g_i (\m{x},\m{y})\m{p}^{k,t+1}$~~ 
% 	   %\EndFor
% 	%	\State $\m{p}^{k,t}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i}^t$
% 	%	\State { $\m{p}^k=\sum_{t=0}^{T-1}\m{p}^{k,t}$}
% 		\EndFor
%  	%	\State $\m{p}_{N'}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i,N'}$ \som{Do we explicitly calculate this, or use HVP (ideal approach)? It should be clarified and we can discuss if needed.}
%  \For {$i \in \mc{S}_{N'+1}$ \textbf{in parallel}} 
%  \State $ \m{x}_{i}= \m{x}_i- \alpha (\nabla_{\m{x}} f_i(\m{x}, \m{y}, \xi_{i})- \frac{N}{\ell_{g,1}}\nabla^2_{\m{xy}}g_i(\m{x},\m{y};{\zeta}_{i,N'+1}) \m{p}_{N'}) $%~~\Comment{via automatic differentiation}
% % \State  $\m{H}_i^{k+1} = \m{H}_i^k + \pi_1 \m{S}_i^k$ and $\m{J}_i^{k+1} = \m{J}_i^k + \pi_2\m{W}_i^k$;
% % %\State Send $\nabla f_i(x^k)$,\; $\mS_i^k \eqdef \cC_i^k(\nabla^2 f_i(x^k) - \mH_i^k)$ and $l_i^k \eqdef \|\mH_i^k - \nabla^2 f_i(x^k)\|_{\rm F}$ to the server
% %\State  $\m{x}^{+}=1/m\sum_{i\in\mathcal{S}}\m{x}_{i}$
% \EndFor
% \State  $\m{x}^{+}=1/|\mc{S}_{N'+1}|\sum_{i\in \mc{S}_{N'+1}} \m{x}_{i}$
% % \EndFor
% \end{algorithmic}
% \end{algorithm}
% }
%  \end{subfigure}
%   \vspace*{-0.15in}
% \end{figure*}



% \begin{figure*}
%  \begin{subfigure}{.47\textwidth}
% \begin{algorithm}[H]
%   \caption*{$\m{x}^{+} ~=~\pmb{\fedout}~(\m{x}, \m{y}, \alpha,N$}
% \begin{algorithmic}[1]
% %\For{$t=T-1,...,0$}
% \State Select $ N'\in \{1, \dots, N\}$ and $\mc{S}_0, \ldots, \mc{S}_{ N'+1} \in \mc{S}$ uniformly at random.
%   \For{$i \in \mc{S}_0$ \textbf{in parallel}} 
%  \State Compute $\nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$
%  \EndFor
%  \State $ \m{p}_0 \leftarrow 1/|\mc{S}_0|\sum_{i\in\mathcal{S}_0} \nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$ 
%  	%	\State $\m{p}_{i,0}\leftarrow \m{p}$
%  		 \For{$n=1,\ldots, N'$}
%  	   % \State Choose $N' \in \{0,\ldots,N-1\}$ randomly and 
% 	%	\For {$i \in \mc{S}$ \textbf{in parallel}} 
% 		\For {$i \in \mc{S}_n$ \textbf{in parallel}} 
% 		 \State $\m{p}_{i,n} \leftarrow (\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_y g_i(\m{x}, \m{y};{\zeta}_{i,n}))\m{p}_{n-1}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y};\xi_j)$}
% 	   \EndFor
% 	   \State $\m{p}_{n}\leftarrow 1/|\mc{S}_n|\sum_{i\in|\mc{S}_n|} \m{p}_{i,n}$
% 	   %\Else 
%  	   %\State $\m{p}_{i}^{k,t}=\m{p}^{k,t+1}-\beta_i \nabla_\m{y}^2  g_i (\m{x},\m{y})\m{p}^{k,t+1}$~~ 
% 	   %\EndFor
% 	%	\State $\m{p}^{k,t}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i}^t$
% 	%	\State { $\m{p}^k=\sum_{t=0}^{T-1}\m{p}^{k,t}$}
% 		\EndFor
%  	%	\State $\m{p}_{N'}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i,N'}$ \som{Do we explicitly calculate this, or use HVP (ideal approach)? It should be clarified and we can discuss if needed.}
%  \For {$i \in \mc{S}_{N'+1}$ \textbf{in parallel}} 
%  \State $ \m{x}_{i}= \m{x}_i- \alpha (\nabla_{\m{x}} f_i(\m{x}, \m{y}, \xi_{i})- \frac{N}{\ell_{g,1}}\nabla^2_{\m{xy}}g_i(\m{x},\m{y};{\zeta}_{i,N'+1}) \m{p}_{N'}) $%~~\Comment{via automatic differentiation}
% % \State  $\m{H}_i^{k+1} = \m{H}_i^k + \pi_1 \m{S}_i^k$ and $\m{J}_i^{k+1} = \m{J}_i^k + \pi_2\m{W}_i^k$;
% % %\State Send $\nabla f_i(x^k)$,\; $\mS_i^k \eqdef \cC_i^k(\nabla^2 f_i(x^k) - \mH_i^k)$ and $l_i^k \eqdef \|\mH_i^k - \nabla^2 f_i(x^k)\|_{\rm F}$ to the server
% %\State  $\m{x}^{+}=1/m\sum_{i\in\mathcal{S}}\m{x}_{i}$
% \EndFor
% \State  $\m{x}^{+}=1/|\mc{S}_{N'+1}|\sum_{i\in \mc{S}_{N'+1}} \m{x}_{i}$
% % \EndFor
% \end{algorithmic}
% \end{algorithm}
%  \end{subfigure}
%   \hspace*{0.03in}
%  \begin{subfigure}{.5\textwidth}
% \begin{algorithm}[H]
%   \caption*{$\m{x}^{+} ~=~\pmb{\fedout}~(\m{x}, \m{y}, \alpha,N$ }
% \begin{algorithmic}[1]
% %\For{$t=T-1,...,0$}
% \State Select $ N'\in \{1, \dots, N\}$ and $\mc{S}_0, \ldots, \mc{S}_{ N'+1} \in \mc{S}$ uniformly at random.
%   \For{$i \in \mc{S}_0$ \textbf{in parallel}} 
%  \State Compute $\nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$
%  \EndFor
%  \State $ \m{p}_0 \leftarrow 1/|\mc{S}_0|\sum_{i\in\mathcal{S}_0} \nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$ 
%  	%	\State $\m{p}_{i,0}\leftarrow \m{p}$
%  		 \For{$n=1,\ldots, N'$}
%  	   % \State Choose $N' \in \{0,\ldots,N-1\}$ randomly and 
% 	%	\For {$i \in \mc{S}$ \textbf{in parallel}} 
% 		\For {$i \in \mc{S}_n$ \textbf{in parallel}} 
% 		 \State $\m{p}_{i,n} \leftarrow (\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_y g_i(\m{x}, \m{y};{\zeta}_{i,n}))\m{p}_{n-1}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y};\xi_j)$}
% 	   \EndFor
% 	   \State $\m{p}_{n}\leftarrow 1/|\mc{S}_n|\sum_{i\in|\mc{S}_n|} \m{p}_{i,n}$
% 	   %\Else 
%  	   %\State $\m{p}_{i}^{k,t}=\m{p}^{k,t+1}-\beta_i \nabla_\m{y}^2  g_i (\m{x},\m{y})\m{p}^{k,t+1}$~~ 
% 	   %\EndFor
% 	%	\State $\m{p}^{k,t}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i}^t$
% 	%	\State { $\m{p}^k=\sum_{t=0}^{T-1}\m{p}^{k,t}$}
% 		\EndFor
%  	%	\State $\m{p}_{N'}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i,N'}$ \som{Do we explicitly calculate this, or use HVP (ideal approach)? It should be clarified and we can discuss if needed.}
%  \For {$i \in \mc{S}_{N'+1}$ \textbf{in parallel}} 
%  \State $ \m{x}_{i}= \m{x}_i- \alpha (\nabla_{\m{x}} f_i(\m{x}, \m{y}, \xi_{i})- \frac{N}{\ell_{g,1}}\nabla^2_{\m{xy}}g_i(\m{x},\m{y};{\zeta}_{i,N'+1}) \m{p}_{N'}) $%~~\Comment{via automatic differentiation}
% % \State  $\m{H}_i^{k+1} = \m{H}_i^k + \pi_1 \m{S}_i^k$ and $\m{J}_i^{k+1} = \m{J}_i^k + \pi_2\m{W}_i^k$;
% % %\State Send $\nabla f_i(x^k)$,\; $\mS_i^k \eqdef \cC_i^k(\nabla^2 f_i(x^k) - \mH_i^k)$ and $l_i^k \eqdef \|\mH_i^k - \nabla^2 f_i(x^k)\|_{\rm F}$ to the server
% %\State  $\m{x}^{+}=1/m\sum_{i\in\mathcal{S}}\m{x}_{i}$
% \EndFor
% \State  $\m{x}^{+}=1/|\mc{S}_{N'+1}|\sum_{i\in \mc{S}_{N'+1}} \m{x}_{i}$
% % \EndFor
% \end{algorithmic}
% \end{algorithm}
%  \end{subfigure}
%   \vspace*{-0.15in}
% \end{figure*}

% \begin{algorithm}[t]
% \caption{~$\m{x}^{+} ~=~\pmb{\fedout}~(\m{x}, \m{y}, \alpha,N$ )
% %\colorbox{red!30}{\pmb{$\fedblo$}}, \colorbox{green!30}{\pmb{$\fedminmax$}}, and \colorbox{blue!20}{\pmb{$\fedcomp$}} 
% }
% \label{alg:fedinn}
% \begin{algorithmic}[1]
% %\For{$t=T-1,...,0$}
% \State Select $ N'\in \{1, \dots, N\}$ and $\mc{S}_0, \ldots, \mc{S}_{ N'+1} \in \mc{S}$ uniformly at random.
%   \For{$i \in \mc{S}_0$ \textbf{in parallel}} 
%  \State Compute $\nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$
%  \EndFor
%  \State $ \m{p}_0 \leftarrow 1/|\mc{S}_0|\sum_{i\in\mathcal{S}_0} \nabla_y f_i(\m{x}, \m{y}; \xi_{i,n})$ 
%  	%	\State $\m{p}_{i,0}\leftarrow \m{p}$
%  		 \For{$n=1,\ldots, N'$}
%  	   % \State Choose $N' \in \{0,\ldots,N-1\}$ randomly and 
% 	%	\For {$i \in \mc{S}$ \textbf{in parallel}} 
% 		\For {$i \in \mc{S}_n$ \textbf{in parallel}} 
% 		 \State $\m{p}_{i,n} \leftarrow (\m{I}-\frac{1}{\ell_{g,1}}\nabla^2_y g_i(\m{x}, \m{y};{\zeta}_{i,n}))\m{p}_{n-1}$% \Comment{$\m{X}_{i,j} := \nabla^2_y g_i(\m{x}, \m{y};\xi_j)$}
% 	   \EndFor
% 	   \State $\m{p}_{n}\leftarrow 1/|\mc{S}_n|\sum_{i\in|\mc{S}_n|} \m{p}_{i,n}$
% 	   %\Else 
%  	   %\State $\m{p}_{i}^{k,t}=\m{p}^{k,t+1}-\beta_i \nabla_\m{y}^2  g_i (\m{x},\m{y})\m{p}^{k,t+1}$~~ 
% 	   %\EndFor
% 	%	\State $\m{p}^{k,t}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i}^t$
% 	%	\State { $\m{p}^k=\sum_{t=0}^{T-1}\m{p}^{k,t}$}
% 		\EndFor
%  	%	\State $\m{p}_{N'}= 1/m\sum_{i\in\mathcal{S}} \m{p}_{i,N'}$ \som{Do we explicitly calculate this, or use HVP (ideal approach)? It should be clarified and we can discuss if needed.}
%  \For {$i \in \mc{S}_{N'+1}$ \textbf{in parallel}} 
%  \State $ \m{x}_{i}= \m{x}_i- \alpha (\nabla_{\m{x}} f_i(\m{x}, \m{y}, \xi_{i})- \frac{N}{\ell_{g,1}}\nabla^2_{\m{xy}}g_i(\m{x},\m{y};{\zeta}_{i,N'+1}) \m{p}_{N'}) $%~~\Comment{via automatic differentiation}
% % \State  $\m{H}_i^{k+1} = \m{H}_i^k + \pi_1 \m{S}_i^k$ and $\m{J}_i^{k+1} = \m{J}_i^k + \pi_2\m{W}_i^k$;
% % %\State Send $\nabla f_i(x^k)$,\; $\mS_i^k \eqdef \cC_i^k(\nabla^2 f_i(x^k) - \mH_i^k)$ and $l_i^k \eqdef \|\mH_i^k - \nabla^2 f_i(x^k)\|_{\rm F}$ to the server
% %\State  $\m{x}^{+}=1/m\sum_{i\in\mathcal{S}}\m{x}_{i}$
% \EndFor
% \State  $\m{x}^{+}=1/|\mc{S}_{N'+1}|\sum_{i\in \mc{S}_{N'+1}} \m{x}_{i}$
% % \EndFor
% \end{algorithmic}
% \label{alg:fedopt}
% \end{algorithm} 

==> sec/gpt4table.tex <==
\begin{table}[t]%\vspace{pt}
\setlength\arrayrulewidth{1.1pt}
\centering
\begin{tabular}{l l|c|c| }
\multicolumn{4}{c}{} \
\cline{3-4}
& \textbf{} & \textbf{Convergence } & \textbf{Communication} \
& & \textbf{ Rate} & \textbf{Complexity}\
\cline{3-4}

\multicolumn{1}{c}{ } &\multicolumn{3}{c}{\large{ Stochastic Multi-Sequence Approximation}} \\
\cline{2-4}
\multicolumn{1}{c}{ }&\multicolumn{1}{|l|}{\textbf{TTSA} ($N= 1$) }& $ \frac{ 1}{R}+ \frac{\sigma^2}{R}$ & N.A. \\
\cline{2-4}
\multicolumn{1}{c}{ }&\multicolumn{1}{|l|}{\textbf{STSA} }& $ %\frac{ C_{\m{h}} }{R}+ \frac{\sigma^2}{R}$
\frac{ 1}{R}+ \frac{\sigma^2}{R}$
& N.A.\\
\cline{2-4}
\multicolumn{1}{c}{ }& \multicolumn{1}{|l|}{\textbf{FedMSA} }& %$ \frac{ \tau C_{\m{h}} }{R}+ \frac{C_{\m{h}} L_\m{h}}{\sqrt{K}R} + \frac{\sigma^2}{MKR}$
$\frac{\tau }{R}+ \frac{L_h}{\sqrt{K}R} + \frac{\sigma^2}{MR}$
& $ \tau\epsilon^{-2}$ \\
\cline{2-4}
\\
\multicolumn{1}{c}{ } &\multicolumn{3}{c}{\large{ Application to Federated Bilevel Optimization}} \\
\cline{3-4}
\cline{2-4}
\multicolumn{1}{c}{ }&\multicolumn{1}{|l|}{\textbf{FedNest} }& $\frac{\Delta_f L_f}{R} + \frac{\sigma^2}{\sqrt{R}} $ & $\epsilon^{-4}$
\\
\cline{2-4}
\multicolumn{1}{c}{ } &\multicolumn{1}{|l|}{\textbf{E-AiPOD} }& $\frac{\Delta_f L_f}{R} + \frac{\sigma^2}{\sqrt{R}} $ & $ \epsilon^{-2}/ R^{3/4}$
\\
\cline{2-4}
\multicolumn{1}{c}{ } &\multicolumn{1}{|l|}{\textbf{AdaFBiO} }&$\frac{\Delta_f+ \sigma^2}{R^{2/3}}$ & $ \epsilon^{-2}$
\\
\cline{2-4}
&\multicolumn{1}{|l|}{\textbf{FedBLO} }& $ \frac{ \tau \Delta_f }{R}+ \frac{\Delta_f L_f}{\sqrt{K}R} + \frac{\sigma^2}{MKR}$ & $ {\tau}\epsilon^{-2}$ \
\cline{2-4}

\multicolumn{1}{c}{ } &
\multicolumn{3}{c}{\large{Application to Federated Compositional Optimization}} \\
\cline{2-4}
\multicolumn{1}{c}{ }&\multicolumn{1}{|l|}{\textbf{ComFedL} ($N= 1$) }& $\frac{\Delta_f L_f}{R} + \frac{\sigma^2}{\sqrt{R}} $ & $\epsilon^{-4}$ \\
\cline{2-4}
\multicolumn{1}{c}{ }& \multicolumn{1}{|l|}{\textbf{FedNest} ($N= 1$)}& $\frac{\Delta_f L_f}{R} + \frac{\sigma^2}{\sqrt{R}}$ & $ \epsilon^{-4}$ \\
\cline{2-4}
\multicolumn{1}{c}{ }&\multicolumn{1}{|l|}{\textbf{AdaMFCGD} ($N= 1$) }& $\frac{\Delta_f+ \sigma^2}{R^{2/3}}$ & $ \epsilon^{-2}$\\
\cline{2-4}
\multicolumn{1}{c}{ }&\multicolumn{1}{|l|}{\textbf{FedMCO} ($N\geq 1$)}& $ \frac{ \tau \Delta_f }{R}+ \frac{\Delta_f L_f}{\sqrt{K}R} + \frac{\sigma^2}{MKR}$ & $ {\tau}\epsilon^{-2}$
\\
\cline{2-4}
\end{tabular}
\vspace{-0.1cm}
\caption{\small{ Comparison of \textbf{convergence rate}, \textbf{communication}, and \textbf{oracle complexity} required by different algorithms to attain. ComFedL \cite{huang2021compositional}, AdaMFCGD \cite{huang2022faster}, FedNest~\cite{tarzanagh2022fednest}, E-AiPOD~\cite{xiao2022alternating}, and AdaFBiO~\cite{huang2022fast}, TTSA \cite{hong2020two}, TTS SA\cite{doan2020nonlinear}. The {\colorbox{green}{$\tau$}} factor controls the benefit we can obtain from small heterogeneity.
}}
\label{table:fedmsa:results}
%\vspace{-0.5cm}
\end{table}%\vspace{-0.15cm}

==> sec/neumann_analysis/notation_neu.tex <==






\newcommand{\kz}{\nu}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\vs}{\vspace}
\newcommand{\fnn}{f_{\text{nn}}}
\newcommand{\ff}{f_{\text{nn}}}
\newcommand{\wi}{k_\st}
\newcommand{\fF}[1]{f_{\text{nn},#1}}
\newcommand{\vc}{\text{vec}}
\newcommand{\flin}{f_{\text{lin}}}
\newcommand{\fln}[1]{f_{\text{lin},#1}}
\newcommand{\rest}{\text{rest}}
\newcommand{\exc}[1]{\mathcal{R}_{\text{gap}}(#1)}
\newcommand{\Mb}{\bar{\M}}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}
\newcommand{\bp}{\bar{p}}
\newcommand{\zig}{\nu}
\newcommand{\bh}{\bar{h}}
\newcommand{\al}{\alpha}
\newcommand{\fs}{f^{\Dc}}
\newcommand{\Ncov}{\mathcal{N}_\eps(\Bal)}
\newcommand{\ft}{h}
\newcommand{\ftv}{f^{\Tc\cup\Vc}}
\newcommand{\deff}{h_{\text{eff}}}
\newcommand{\defz}{\bar{h}_{\text{eff}}}
\newcommand{\deft}{\tilde{h}_{\text{eff}}}
\newcommand{\defg}{\bar{h}^{\nabla}_{\text{eff}}}
\newcommand{\defF}{\bar{h}^{\FB}_{\text{eff}}}
\newcommand{\bC}{\bar{C}}
\newcommand{\nt}{n_\mathcal{T}}
\newcommand{\h}{h}
\newcommand{\nv}{n_\mathcal{V}}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\pleq}{\overset{{P}}{\leq}}
\newcommand{\np}{{n\wedge p}}
\newcommand{\KB}{\bar{K}}
\newcommand{\bG}{\boldsymbol{\Gamma}}
\newcommand{\rP}{\stackrel{{P}}{\longrightarrow}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\yb}{\bar{\y}}
\newcommand{\hu}{h}
\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\cmp}{P_{\text{nn}}}
%\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\ba}{\begin{align}}
\newcommand{\ea}{\end{align}}
\newcommand{\bea}[1]{\begin{align}#1\end{align}}
\newcommand{\nrest}{\bar{n}}
\newcommand{\eeq}{\end{equation}}
%\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
%\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\vrn}{\sigma}
\newcommand{\sgt}[1]{\tilde{\sigma}^{(#1)}}
\newcommand{\tsig}{\tilde{\sigma}}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
%\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\laz}{\la_0}
\newcommand{\blaz}{\bar{\la}_0}
\newcommand{\caz}{\la_C}
\newcommand{\saz}{L_\sigma}
\newcommand{\Lat}{\tilde{\Lambda}}
\newcommand{\K}{{K}}

\newcommand{\Aa}{{\mtx{A}}}
\newcommand{\Bb}{{\mtx{B}}}
\newcommand{\N}{{\mtx{N}}}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\btm}{\bigotimes}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\fp}{F}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Hc}{{\cal{H}}}
\newcommand{\Lcz}{{\cal{L}}^{0-1}}
\newcommand{\Lczh}{{\hat{\cal{L}}}^{0-1}}
\newcommand{\Lch}{{\widehat{\cal{L}}}}
\newcommand{\Lcv}[1]{{\cal{L}}^{#1}_{\text{up}}}
\newcommand{\Lct}[1]{{\cal{L}}^{#1}_{\text{low}}}
\newcommand{\Lcb}{{\bar{\cal{L}}}}
\newcommand{\Nc}{{\cal{N}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Dc}{{\cal{D}}}
\newcommand{\Dci}{{\cal{D}}_{\text{init}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Tn}{{T_0}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\Qh}{{\mtx{\hat{Q}}}}
\newcommand{\Qt}{{\mtx{\tilde{Q}}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Hbi}{{\mtx{H}\mtx{I}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\relu}[1]{\phi(#1)}
\newcommand{\one}[1]{{\bm{1}}(#1)}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSii}{{\boldsymbol{{\Sigma}}}_{i,i}}
\newcommand{\bSib}{\bar{{\boldsymbol{{\Sigma}}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\bB}{{\bar{B}}}
\newcommand{\tB}{{\tilde{B}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}

%\newcommand{\M}{{\mtx{M}}}
\newcommand{\gm}{\gamma_m}
%\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\ordet}[1]{{\widetilde{\cal{O}}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{s_{\min}(#1)}}
\newcommand{\smx}[1]{{s_{\max}(#1)}}
\newcommand{\zt}{{\tilde{\vct{z}}}}
\newcommand{\fab}{f^\bal_\bt}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\el}{{\ell}}
\newcommand{\sft}[1]{\text{shift}(#1)}
%\newcommand{\tn}[1]{\|{#1}\|_{\ell_2}}
\newcommand{\nrm}[1]{\|{#1}\|}%_{#2}}
\newcommand{\inr}[1]{\left<#1\right>}
\newcommand{\tone}[1]{\|{#1}\|_{\ell_1}}
\newcommand{\lix}[1]{\|{#1}\|_{\Xc}}
\newcommand{\lif}[1]{\text{dist}_{\FB}({#1})}
\newcommand{\lit}[1]{\text{max}(#1)}%_{\Ttc}
\newcommand{\lia}[1]{\text{avg}(#1)}%
\newcommand{\lin}[1]{\|{#1}\|_{L_\infty}}
\newcommand{\tff}[1]{\|{#1}\|_{\ell_4}}
\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\trow}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Lcg}{\tilde{\Lc}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
\newcommand{\upp}{{\cal{B}}_{\alpha,\Gamma}}
\newcommand{\upz}{{\cal{B}}_{\alpha_0,\Gamma}}
\newcommand{\dpz}{{\cal{D}}_{\alpha_0,\Gamma}}
\newcommand{\dpp}{{\cal{D}}_{\alpha,\Gamma}}
\newcommand{\mpp}{M_{\alpha,\Gamma}}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Al}[1]{\Ac(#1)}
\newcommand{\Alg}[1]{\Ac_g(#1)}
\newcommand{\Acg}{\Ac_g}
\newcommand{\At}{\mathcal{A}}
%\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Acr}{\mathcal{A_\text{ridge}}}
\newcommand{\Bal}{{\boldsymbol{\Delta}}}
\newcommand{\del}{\delta}
\newcommand{\bdel}{\boldsymbol{\delta}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Rcp}{\mathcal{\bar{R}}'}
\newcommand{\Rcb}{\mathcal{N}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bt}{{\boldsymbol{\beta}}}
\newcommand{\bT}{{\boldsymbol{\Theta}}}
\newcommand{\bts}{{\boldsymbol{\beta}_\st}}
\newcommand{\btb}{\bar{\boldsymbol{\theta}}}
\newcommand{\btid}{\boldsymbol{\theta}^\text{ideal}}
\newcommand{\btt}{\tilde{\boldsymbol{\theta}}}
\newcommand{\bal}{{\boldsymbol{\alpha}}}
\newcommand{\bgam}{{\boldsymbol{\gamma}}}
\newcommand{\bab}{{\boldsymbol{\bar{\alpha}}}}
\newcommand{\sbl}[1]{\sigma_{\boldsymbol{\alpha^{(#1)}}}}
\newcommand{\bl}[1]{{\boldsymbol{\alpha}}^{(#1)}}
\newcommand{\blb}[1]{\bar{\boldsymbol{\alpha}}^{(#1)}}
\newcommand{\bah}{{\widehat{\bal}}}
\newcommand{\bas}{{\boldsymbol{\alpha}_\st}}
\newcommand{\bth}{{\boldsymbol{\hat{\beta}}}}
\newcommand{\bPhi}{{\boldsymbol{\Phi}}}
\newcommand{\bbteta}{\widetilde{\boldsymbol{\theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\DD}{{D}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\No}{N}
\newcommand{\Bc}{\mathcal{B}}

\newcommand{\Sci}{\mathcal{S}_{\text{in}}}
\newcommand{\Sco}{\mathcal{S}_{\text{out}}}
\newcommand{\Ect}{\mathcal{S}_{\text{top}}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
%\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\Jt}{\mtx{\tilde{J}}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\Fb}{\vct{F}}
\newcommand{\FB}{\mathbb{F}}
\newcommand{\Ft}{\tilde{\vct{F}}}
\newcommand{\fa}{\tilde{\vct{f}}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\xb}{\vct{\bar{x}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\ist}{i_\st}
\newcommand{\err}[1]{\text{Err}_{\Dc}(#1)}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\tilW}{\widetilde{\mtx{W}}}
\newcommand{\tilw}{\widetilde{\vct{w}}}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
%\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}
%\newcommand{\s}{\vct{s}}
\newcommand{\ab}{\vct{a}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
%\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\Hh}{{\mtx{\hat{H}}}}
\newcommand{\Ht}{{\mtx{\tilde{H}}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\text{{\bf{zm}}}(#1)}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\TVc}{\Tc\cup\Vc}
\newcommand{\Ttc}{\mathcal{T}_{\text{test}}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Fcl}{\mathcal{F}^{\text{lin}}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}


%%YP's macros
\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}{#1}}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
%\newcommand{\m}[1]{{\bf{#1}}}
\newcommand{\xt}{\widetilde{\x}}
\newcommand{\yt}{\widetilde{y}}
\newcommand{\ybt}{\tilde{\y}}
\newcommand{\Xt}{\tilde{\X}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
%\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\wnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\lab}{\bar{\la}}
\newcommand{\avg}[1]{\left< #1 \right>}


\newcommand{\mult}{B^D\bar{M}N}
\newcommand{\liptwo}{20R^3B\nt^2\laz^{-2}(B\nt+1)}
\newcommand{\lipp}{5R^2\sqrt{B^3\nt^3\h}\laz^{-2}\tn{\yT}}
\newcommand{\lips}{6R^3B^2\sqrt{\nt^3\h}\laz^{-2}\tn{\yT}}
\newcommand{\lipl}{5(RB\nt\sqrt{\h}+1)RB\nt\laz^{-2}}
\newcommand{\lip}{\frac{5B^2\tn{\yT}}{\laz^2}}
\newcommand{\lipt}{6R^3B^2\Gamma\sqrt{\nt^3\h}\laz^{-2} \tn{\yT}}
\newcommand{\lipf}{{20R^4B^2\laz^{-2}\Gamma\nt^2\tn{\yT}}}

\newcommand{\lipnn}{120B^4\blaz^{-2}\Gamma(\nt^2+\nv^2) \tn{\yT}}
\newcommand{\bL}{\bar{L}}
\newcommand{\scl}{M}
\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
%\newcommand{\x}{\vct{x}}
\newcommand{\xx}[1]{\vct{x}^{(#1)}}
\newcommand{\rbb}{\vct{\widetilde{r}}}
%\newcommand{\y}{\vct{y}}
\newcommand{\yT}{\vct{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Ww}[1]{\mtx{W}^{(#1)}}
\newcommand{\Wt}{\tilde{\mtx{W}}}
\newcommand{\Wc}{{\cal{W}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\definecolor{emmanuel}{RGB}{255,127,0}
\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\Kbb}{{\mtx{\bar{K}}}}
\newcommand{\Kbh}{{\widehat{\mtx{K}}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
%\newcommand{\Var}{\textrm{Var}}
\newcommand{\Cov}[1]{\textrm{Cov}[#1]}
%\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
%\newcommand{\E}{\operatorname{\mathbb{E}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

%\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eb}{\vct{e}}
\renewcommand{\i}{\imath}


% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\OpId}{\mathcal{I}}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}
\newcommand{\bR}{{\bar{R}}}

\newcommand{\calF}{\mathcal{I}}
\newcommand{\calS}{\mathcal{N}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}


==> sec/prelim.tex <==



%\subsection{}  



% \begin{algorithm}[t]
%   \caption{$\m{s}_N=~\pmb{\fedimvp}~(N)$:} %Federated approximate inverse-Hessian product
% \begin{algorithmic}[1]
% \State Select $\Sc_0,\Sc_1, \ldots, \Sc_{ N'} \in \Sc$ UAR.
%   \For{$i \in \Sc_0$ \textbf{in parallel}} 
%  \State $\m{v}_{i,0} =\m{b}_i$
%  \EndFor
%  \State $ \m{v}_0 = \frac{1}{\eta}  |\Sc_0|^{-1}\sum_{i\in\mathcal{S}_0} \m{p}_{i,0}$  and  $\m{s}_0=\m{v}_0$
% % \State Select i.i.d.~$\Sc_1, \ldots, \Sc_{N} \in \Sc$ each drawing $B$ i.i.d.~clients with replacement% i.i.d.~Bernoulli$(p)$
% %\State $\m{v}_0=L\m{v}$, 
% \For{$n=1,\ldots, N$}
% 		\For {$i \in \Sc_n$ \textbf{in parallel}} 
% 		 \State $\m{v}_{i,n} = \left(\m{I}-\eta \m{A}_{i,n})\right)\m{v}_{n-1}$
% 	   \EndFor
% 	   \State $\m{v}_{n}=|\Sc_n|^{-1}\sum_{i\in\Sc_n} \m{v}_{i,n}$ 
% 	   \State $\m{s}_n=\m{s}_{n-1}+\m{v}_n$
% 		\EndFor	
% \end{algorithmic}\label{fedihgp_algo}
% \end{algorithm}


%   
%We emphasize that \eqref{eqn:lsys:main} is different form the following least-square problem that is widely studied in literature:

% \section{Implicit Deep Learning}\label{sec:idl}
% Consider solving a fixed-point equation in some single ``state'' vector $x \in \mb{R}^n$. That is, for a given input vector $u$, the predicted vector is
% \begin{subequations}\label{eq:pred-rule-top}
% \begin{align}
%   \hat{y}(u) &=Cx+Du   \label{eq:pred-rule} \\
%   x &= \phi(Ax+Bu)  \label{eq:eq-eq} 
% \end{align}
% \end{subequations}
% where $\phi \::\: \mb{R}^n \rightarrow \mb{R}^n$ is a nonlinear vector map (the ``activation'' map), and matrices $A,B,C,D$ contain model parameters. In IDL training \citep{el2021implicit} we are given an input data matrix $U = [u_1,\ldots,u_m] \in \mb{R}^{p \times m}$ and response matrix $Y = [y_1, \ldots, y_m] \in \mb{R}^{q \times m}$, and seek to fit a model of the form~\cref{eq:pred-rule}, with $A$ well-posed with respect to $\phi$, which we assume to be a blockwise Lipschitz map.  We note that the rule~\cref{eq:pred-rule}, when applied to a collection of inputs $(u_i)_{1 \le i \le m}$, can be written in matrix form, as
% \[
% \hat{Y}(U) = CX+DU , \mbox{ where } X = \phi(AX+BU).
% \]
% where $U = [u_1,\ldots,u_m] \in \mb{R}^{p \times m}$, and $\hat{Y}(U) = [\hat{y}(u_1), \ldots, \hat{y}(u_m)] \in \mb{R}^{q \times m}$. 

% In this case, a federated training problem has the following form
% \begin{equation}\label{eq:training-pb}
% \min_{A,B,C,D,X} \:\frac{1}{m}\sum_{i=1}^m f_i(Y,CX+DU) + {\cal P} (A,B,C,D) ~:~ X = \phi(AX+BU),
% \end{equation}
% In the above, $f_i$ is a loss function for $i$-th client, and ${\cal P}$ is a convex penalty function. In this case, the gradient is given by  the following closed form evaluation of gradients for ($A, B, C, D$):
% $$
%  \frac{1}{m}\sum_{i=1}^m
%  \begin{pmatrix}
% \nabla_A  f_i &
% \nabla_B  f_i \\
% \nabla_C f_i &
% \nabla_D f_i \\
% \end{pmatrix} = \begin{pmatrix}
% \nabla_z f \\
% \nabla_{\hat{y}} f
% \end{pmatrix}
% \begin{pmatrix}
% x \\ u 
% \end{pmatrix}^\top.
% $$

 
 
 


% \section{Stochastic Federated Linear System Solvers with Vector Costs}\label{sec FLS}

% To present our results, let us fix the notation and setting. For an integer $k$, denote $[k]=\{1,2,\dots,k\}$. Let $m$ be the number of clients and $\Sc:=[m]$ denote the set of all clients. Recall that we have $\m{A}_{i} \in \mb{R}^{p \times p }$, $\m{b}_{i} \in \mb{R}^{p }$ for all $i \in \Sc$. We consider a general stochastic oracle model: Access to $(\m{A}_i, \m{b}_i)$ is via stochastic sampling, i.e., $\m{A}_i := \mb{E}_{\xi \sim \mc{C}_i}\left[\m{A}_i(\xi)\right]$ and $\m{b}_i := \mb{E}_{\zeta \sim \mc{D}_i}\left[\m{b}_i(\zeta)\right]$ where $(\xi, \zeta)\sim(\mc{C}_i, \mc{D}_i)$ are sampling distribution for the $i^{\text{th}}$ client. We emphasize that for $i \neq j$, $(\m{A}_i,\m{b}_i,\mc{C}_i, \mc{D}_i)$ and $(\m{A}_j,\m{b}_j,\mc{C}_j, \mc{D}_j)$ can be different (objective heterogeneity). $\tn{\cdot}$ denotes spectral norm for matrices and $\ell_2$ norm for vectors.

% \noindent \textbf{\emph{Assumptions.}} Throughout, we make the following assumptions on~\eqref{eqn:lsys:main}.
% %
% \begin{assumption}\label{assu:lsys:a} 
% For all $i \in \Sc:=[m]$, $\m{A}_i$ is a symmetric positive definite matrix satisfying $L\Iden\succeq \A_i\succeq \mu \Iden$ for some $L\geq \mu>0$.
% \end{assumption}
% Throughout, we use $\kappa=L/\mu$ to denote the condition number of System~\eqref{eqn:lsys:main}.
% \begin{assumption}[Stochastic samples]\label{assu:lsys:bound:var}
% For all $i \in [m]$:
% \begin{enumerate}[label={\textnormal{\textbf{(B\arabic*})}}]
% \vspace{-.15cm}
% \item $\m{A}_i(\xi)$ and $\m{b}_i(\zeta)$ are unbiased estimators of $\m{A}_i$ and $\m{b}_i$, respectively; and
% \vspace{-.15cm}
% %$\mb{E}_{\xi}[\nabla f_i(\m{z};\xi)]=\nabla f_i(\m{z})$, $\mb{E}_{\zeta}[\nabla g_i(\m{z};\zeta)]=\nabla g_i(\m{z})$, $\mb{E}_{\zeta}[\nabla^2 g_i(\m{z}, \zeta)=\nabla g_i(\m{z})]$
% %are unbiased estimators of $\nabla f_i(\m{z})$, $\nabla g_i(\m{z})$, and $\nabla^2g_i(\m{z})$, respectively;
% \item Their variances are bounded, i.e., $\mb{E}_{\xi}[\|\m{A}_i(\xi)-\m{A}_i\|^2] \leq \sigma_\m{A}^2$ and    $\mb{E}_{\zeta}[\|\m{b}_i(\zeta) -\m{b}_i\|^2] \leq \sigma_{\m{b}}^2$ for some $\sigma_{\m{A}}$ and $\sigma_{\m{b}}$. When $\sigma_{\m{A}}=\sigma_{\m{b}}=0$, we refer to the samples as \emph{deterministic}. 
% \end{enumerate}
% \end{assumption}
 



% In this section, we develop our proposed FL algorithm for solving \eqref{eqn:lsys:main}. We denote the solution of \eqref{eqn:lsys:main} by $\m{z}^{\star} = \m{A}^{-1}\m{b}$, where $\m{A} =1/m\sum_{i=1}^m \m{A}_i$ and $\m{b} =1/m\sum_{i=1}^m \m{b}_i$. In order to approximate the \textit{stochastic} matrix inverse in general FL setting, we consider a \emph{Neumann series} expansion of linear operators, which we now recall. Let $\m{I}$ denote the $p\times p$ identity matrix. Then, for any $\eta \leq  1/ \|\m{A}\| $, we have 
% \begin{equation}\label{eq:neumann1}
%     \m{A}^{-1} = \eta \sum_{k=0}^\infty (\m{I}-\eta \m{A})^k~.
% \end{equation}
% A truncated version of \eqref{eq:neumann1} is widely used in non-FL stochastic nonlinear optimization \citep{agarwal2017second,ghadimi2018approximation,hong2020two}.
% % In particular, a sufficient condition for the convergence of the Neumann series is $\|\m{A}\| < 1$ where $\|\cdot\|$ is the operator norm. 
% %\subsection{Federated Estimator~I: Neumann Approximation} 
% Closer to us, for FL, \citet{tarzanagh2022fednest} proposed a client sampling strategy to estimate $\m{z}^*$ in an efficient distributed stochastic manner. In particular, given $N \in \mb{N}$, they select $N' \in \{0 \ldots, N-1\}$ uniformly at random. Then, they estimate $\z$ via $\z\approx \z_{N'}$ over $N'$ communication rounds where
% %and $\Sc_0, \ldots, \Sc_{ N'} \subset \Sc$
% \begin{align}
%     \m{z}_{N'} = N\eta \prod_{n=1}^{N'} \Big (\m{I} - \frac{\eta}{m} \sum_{i=1}^{m} \m{A}_i(\xi_{i}^n) \Big) \m{v}_0,~~~\textnormal{and}~~~\m{v}_0=m^{-1}\sum_{i\in\Sc} \m{b}(\zeta_{i}^0).
%     \label{eq:hessinv:est}
% \end{align}
% %\begin{wrapfigure}{r}{0.4\textwidth}
% %\begin{minipage}{0.4\textwidth}
% %\vspace{-8mm}
% \begin{algorithm}[t]
%   \caption{$\m{v}^{+}=~\pmb{\mc{A}}~(\bb,\vb,\eta)$} %Federated approximate inverse-Hessian product
% \begin{algorithmic}[1]
% % \State %$\m{v}^0=\m{s}^0$
%   %\State $\m{b}=m^{-1}\sum_{i\in\Sc}\m{b} (\zeta_{i}^n) $
% %\For{$n=1,\ldots, N$}
%   \State $\m{s}= m^{-1}\sum_{i\in\Sc}\m{A}_i(\xi_{i,0}) \m{v}-\m{b}$
%   \State $\m{v}_{i,0} =\m{v}$ and $\eta_i \in (0,\eta]$  
%   \For {$\nu=0,\ldots,\tau_i-1$} 
% 		 \State $\m{v}_{i,\nu+1} = (\m{I}-\eta_i\m{A}_i(\xi_{i,\nu}))\m{v}_{i,\nu}$
% 		 \State $~~~~~~~~~~-\eta_i \left(\m{s} -\m{A}_i(\xi_{i,\nu})\m{v}\right)$
% 	   \EndFor
% 	   \State $\m{v}^{+}=m^{-1}\sum_{i\in\Sc} \m{v}_{i,\tau_i}$
% %		\EndFor	
% \end{algorithmic}\label{alg:fed:richardson}
% \end{algorithm}
%  %\vspace{-15mm}
%  %\end{minipage}
%  %\end{wrapfigure}
% % \begin{wrapfigure}{r}{0.5\textwidth}
% % \begin{minipage}{0.5\textwidth}
% % \vspace{-8mm}
% % \begin{algorithm}[H]
% %   \caption{$\m{v}^{+}=~\pmb{\mc{A}}~(\m{v},\eta)$} %Federated approximate inverse-Hessian product
% % \begin{algorithmic}[1]
% % % \State %$\m{v}^0=\m{s}^0$
% %   %\State $\m{b}=m^{-1}\sum_{i\in\Sc}\m{b} (\zeta_{i}^n) $
% % %\For{$n=1,\ldots, N$}
% %   \State $\m{s}^{n}= m^{-1}\sum_{i\in\Sc}\m{A}_i(\xi_{i}^{n}) \m{v}^{n}-\m{b}$
% %   \State $\m{v}_{i,0}^{n} =\m{v}^{n}$ and $\eta_i \in (0,\eta]$  
% %   \For {$\nu=0,\ldots,\tau_i-1$} 
% % 		 \State $\m{v}_{i,\nu+1}^{n} = (\m{I}-\eta_i\m{A}_i(\xi_{i,\nu}^n))\m{v}_{i,\nu}^{n}$
% % 		 \State $~~~~~~+ \eta_i \m{A}_i(\xi_{i,\nu}^n)\m{v}^{n}-\eta_i s^{n}$
% % 	   \EndFor
% % 	   \State $\m{v}^{+}=m^{-1}\sum_{i\in\Sc} \m{v}_{i,\tau_i}^{n}$
% % %		\EndFor	
% % \end{algorithmic}\label{fed:vr:richardson}
% % \end{algorithm}
% %  %\vspace{-15mm}
% %  \end{minipage}
% %  \end{wrapfigure}
% % %However, in expectation, it requires $\E[N']=N/2$ round of communication. 
% %In contrast, over $N$ rounds, one can calculate $\$
% %The above estimator has the disadvantage that in a single sample it incorporates only \textit{one term} of the Taylor series \eqref{eq:neumann1}.  Prima facie in order to estimate all the terms to a certain level one needs a quadratically growing number of samples which worsens the sample complexity. 
% This estimation strategy has two drawbacks leading to high-variance and inefficient communication. This is due to two issues: First, this strategy samples only a \textit{single element} of the first $N$ terms of the Neumann series \eqref{eq:neumann1}. It is wasteful and high-variance because even if $N'+1$ terms are calculated (from $\z_0$ to $\z_{N'}$), only one is chosen and rest are discarded. Secondly, clients don't use any local iterations. In practice, one can dramatically reduce communication rounds $N$ by running local iterations. We address the first issue by proposing a better estimator that uses the sum of $N$ terms of \eqref{eq:neumann1}. To do so, we note that we can solve \eqref{eqn:lsys:main} via the following distributed recurrence relation starting from $\vb_0$ of \eqref{eq:hessinv:est}
% %  Specifically, given $N \in \mb{N}$, we select $N' \in \{0 \ldots, N-1\}$ and $\Sc_0, \ldots, \Sc_{ N'} \in \Sc$ UAR, and define 
% \begin{align}\label{eqn:witho:local}
% %\m{v}^1 =m^{-1}\sum_{i\in\Sc} \m{b} (\zeta_{i}^1) ~~~\textnormal{and}~~~
% \m{v}^{n+1}= \eta \m{v}^1+\Big(\m{I} -\frac{\eta}{ m}\sum_{i=1}^{m} \m{A}(\xi_{i}^n) \Big)\m{v}^{n}.
% %\label{eq:hessinv:est}
% \end{align}
% %\ps{Should the first term in update of $\m{v}^{n+1}$ instead be $\eta^{-1} \m{v}^1$?}
% It can be easily seen that $\mb{E} [\m{v}^n] \rightarrow \m{z}^*$ as $n \rightarrow \infty$, providing us with an unbiased estimator in the limit. Note that the above procedure can be considered as a distributed variant of Richardson Iteration \citep{varga1962iterative} for solving stochastic linear systems.   Algorithm~\ref{alg:fed:richardson} gives a single round of our proposed FL approach to tackle heterogeneity in \eqref{eqn:lsys:main} and improve communication rounds of \eqref{eqn:witho:local}. Specifically, in each round, starting from a common global model $\m{v}_{i,0}=\m{v}$, each client $i$ performs $\tau_i$ local steps (in parallel):
% \begin{align}\label{eqn:update1:fedout}
%     \m{v}_{i,\nu +1}=\big(\m{I}-\eta_i\m{A}_i(\xi_{i,\nu})\big)\m{v}_{i,\nu} -\eta_i \big(\m{s}-\m{A}_i(\xi_{i,\nu})\m{v}\big)
% \end{align}
% and then the server aggregates local models via $\m{v}^{+}=m^{-1} \sum_{i\in \Sc} \m{v}_{i,\tau_i}$. Here, $\eta_i \in (0,\eta]$ is the local stepsize and $\m{s}=m^{-1}\sum_{i\in\Sc}\m{A}_i(\xi_{i})\m{v}-\m{b}$.
% The key features of update \eqref{eqn:update1:fedout} is exploiting past $\m{v}$ and $\m{s}$ to account for heterogeneity. Indeed, the ideal update in Algorithm~\ref{alg:fed:richardson} would perform  $\m{v}_{i,\nu +1}=\eta_i \m{v}+(\m{I}-\eta_i \sum_{i=1}^m\m{A}_i(\xi_{i,\nu}))\m{v}_{i,\nu}$. But this requires each client $i$ to have access to the global coefficient matrix $\m{A}$--which it does not, since clients do not communicate between rounds. To overcome this issue, each client $i$ uses $\m{s}$ from the beginning of each round as a guiding direction in its local update rule. However, since $\m{s}$ is computed using previous $\m{A}_i(\xi)$, client $i$ makes a correction by subtracting off the stale estimate $\m{A}_i(\xi_{i,\nu})\m{v}$ and adding its own \emph{local} estimate $\m{A}_i(\xi_{i,\nu})\m{v}_{i,\nu}$. Our local update rule in Step~4 of Algorithm~\ref{alg:fed:richardson} is precisely of this form.
%  \ps{In the notation above, $i$ is the client index, and $n, \nu$ are, respectively, the iteration index and the local update within an iteration index. I think it would be better to club $n, \nu$ in subscript/superscript, to make easier to read. For example, $\m{v}_{i}^{n,\nu}$.}

% \subsection{The Homogeneous Setting}
% \begin{theorem}\label{thm:fedIMVP:homo}
% Suppose Assumptions~\ref{assu:s:f} and \ref{assu:s:bound:var} hold. Then, 
% % \begin{align*}
% % % \E \|\m{v}^N -\m{v}_0\| &\leq c\cdot \left(\frac{HB^2}{\nu N} + \frac{\sigma B}{\sqrt{M\nu N}}\right) \\
% % \E \left[\|\m{v}^N -\m{v}_0\|\right] &\leq c\cdot \left(\Delta\exp\left(-\frac{c'\lambda \nu N}{H}\right) + \frac{\sigma^2}{\lambda M\nu N}\right).
% % \end{align*}
% % Then, the following inequalities holds:
% \begin{align}
% 	&&\mb{E}\left[\|\m{v}^{N}-\m{v}^{\star}\|^2\right] \leq & (1-\eta\mu_g)^{\nu N} \|\m{v}-\m{v}^{\star}\|^2 +  
% 			\eta^2 \left(\frac{\sigma_A^2}{M}\|\m{v}^{\star}\|^{2} + \frac{3\nu N}{\eta\mu_g}\frac{\sigma_b^2}{M}\right)  \left(\frac{\nu N}{\eta \mu_g}\right).
% \end{align}

% \end{theorem}

% \begin{theorem}[\textbf{Linear-Quadartic Rate}]\label{thm:fednewton}
% Suppose Assumptions~\ref{assu:s:f} and \ref{assu:s:bound:var} hold.  %Further, assume $\alpha_i^k=\alpha_k/\tau_i$ for all $ i \in \mathcal{S}$, where
% Then, 
% 	\begin{equation}  \label{capsule}
% 	\E \left[\|\m{x}^{k+1}-\m{x}^*\|\right] \leq C_1 \|\m{x}^k -\m{x}^*\|^2+\left( \frac{C_2}{\sqrt{\beta}} +C_3 \theta^r \right) \|\m{x}^k-\m{x}^*\| + C_4,
% 	\end{equation}
% 	where    
% 	\begin{equation}   \label{c3}
% 	C_1=, \quad C_2 =, \quad   
% 	C_3 = , C_4= \quad \theta=, \quad
% 	\delta(\beta)= .
% 	\end{equation}
% \end{theorem}
% %
% %
% \subsection{The Homogeneous Setting}
% \begin{definition}[FLS heterogeneity]
% We say that $\{\m{A}_i\}_{i=1}^m$ are $\omega$--heterogeneous if $\textnormal{sup}_{i\in \Sc}\|\m{A}_{i}-\m{A}\| \leq \omega$.  
% \end{definition}
%     Note that the above assumption is less restrictive than the widely used first order heterogeneity \cite{wang2022unreasonable}. We emphasize that even if $\{f_i\}_{i=1}^m$ are $L$-smooth, the Hessian matrices $\m{A}_i= \nabla^2 f_i $ may not satisfy the above assumption \footnote{ $\omega$ must be smaller than $2L$}.  
% %\ps{Given $L$-smoothness of $\{ f_i \}_i$, we already have that $\| \nabla^2 f_{i}(\m{x}) \| \leq L$ for all $i, \m{x}$. Do we need this assumption then?}

% \begin{lemma}[Deterministic sampling]\label{deter lem} Suppose sampling is deterministic and run Algorithm \ref{alg:fed:richardson} for $N$ communication rounds. Each round admits input $\vb_n$ and returns $\vb_{n+1}$. Set residual $\rb_n=\vb_n-\A^{-1}\bb$. We have that
% \[
% \rb_N= \Big[\frac{1}{m}\sum_{i=1}^m\Big((\Iden-\eta \A_i)^\tau+\eta \sum_{t=0}^{\tau-1}(\Iden-\eta \A_i)^t(\A_i-\A)\Big) \Big]^N\rb_0.
% \]
% Taking $\ell_2$ norms of both sides and applying standard upper bounds, for $\eta\leq 1/L$
% \begin{align*}
% \tn{\rb_N}&\leq \Big((1-\eta\mu)^\tau+\eta \Big\|\frac{1}{m}\sum_{i=1}^m\sum_{t=0}^{\tau-1}(\Iden-\eta \A_i)^t(\A_i-\A)\Big\| \Big)^N\tn{\rb_0}\\
% &\leq\Big((1-\eta\mu)^\tau+ (1-(1-\eta\mu)^\tau) \omega/\mu\Big)^N\tn{\rb_0}.
% \end{align*}
% %Thus, the number of communication rounds for $\eps$-error grow proportional to $\log(\eps)/\log\|\Iden-\M\A\|$.
% \end{lemma}

% \red{\textbf{TODO:} Characterize the largest $\tau$ (as a function of $\omega$) till which we achieve the near-optimal $\tn{\rb_N}\lesssim (1-\eta\mu)^{c N\tau}\tn{\rb_0}$ rate for a constant $c>0$.}

% \begin{proof} We consider a single round from which $N$ round follows immediately. Set $\vb_{i,0}=\vb_0=\vb$ and $\rb_{i,t}=\vb_{i,t}-\vb_\st$ with $\vb_\st=\A^{-1}\bb$. The client $i$ runs iterations $0\leq t\leq \tau-1$
% \begin{align*}
% \vb_{i,t+1}=(\Iden-\eta \A_i)\vb_{i,t}+\eta\A_i\vb-\eta \A\vb+\eta \A\vb_\st
% \end{align*}
% Subtracting $\vb_\st$ from both sides, this implies%and setting $\rb_{i,t}=\vb_{i,t}-\vb_\st$
% \begin{align*}
% \rb_{i,t+1}&=\rb_{i,t}-\eta \A_i\vb_{i,t}+\eta\A_i\vb-\eta \A\rb_0\\
% &=\rb_{i,t}-\eta \A_i\rb_{i,t}+\eta\A_i\rb_0-\eta \A\rb_0\\
% &=(\Iden-\eta\A_i)\rb_{i,t}+\eta(\A_i-\A)\rb_0.
% %&=(\Iden-\eta \A)\rb_{i,\tau}-\eta (\A_i-\A)(\rb_{i,\tau}-\rb_{0,\tau}).
% \end{align*}
% After $\tau$ iterations, we have the closed form expression
% \begin{align*}
% \rb_{i,\tau}&=(\Iden-\eta \A_i)^\tau\rb_{0}+\eta \sum_{t=0}^{\tau-1}(\Iden-\eta \A_i)^t(\A_i-\A) \rb_{0}\\
% &=\left[(\Iden-\eta \A_i)^\tau+\eta \sum_{t=0}^{\tau-1}(\Iden-\eta \A_i)^t(\A_i-\A) \right]\rb_{0}.
% \end{align*}
% This concludes the proof after plugging the above equation into $\hat{\rb}=\frac{1}{m}\sum_{i=1}^m \rb_{i,\tau}$.
% \end{proof}

% \begin{corollary}[Simplification with $\tau\rightarrow\infty$] Consider the setting of Lemma \ref{deter lem}. Set mean-of-inverse matrix $\M=\frac{1}{m}\sum_{i=1}^m\A_i^{-1}$. After $N$ rounds of Algorithm \ref{local_Neumann_round} with deterministic sampling and $\tau=\infty$ iterations, we have 
% \[
% \tn{\vb^N-\A^{-1}\bb}\leq (\Iden-\M\A)^N\tn{\vb^0-\A^{-1}\bb}
% \]
% Thus, the number of communication rounds required for achieving $\eps$-error grow proportional to $\log(\eps)/\log\|\Iden-\M\A\|$.
% \end{corollary}

% %
% \begin{theorem}
% For each $i \in \Sc$, let $\eta_i$ the outcome of Algorithm \ref{fedihgp_algo}
% % obeys
% % \begin{equation*}
% % \tau_i \geq 1,~~~~\alpha_i=\frac{\alpha}{\tau_i},~~~~\beta_i=\frac{\beta}{\tau_i},~~~~\forall i \in \mathcal{S},    
% % \end{equation*}
% % where  $0<\beta <  \min\big(1/(6\ell_{g,1}),1\big)$ and $\alpha$ is some positive constant. Then, \fedinn 
% guarantees: 
% \begin{align}
%     \mb{E}\left[\left\|\m{v}^{(N)}-\m{v}^\star\right\|^2\right]& \leq  \left(1-  \frac{{\eta} \mu_g}{2} \right)^N \mb{E}\left[\left\| \m{v}^1- \m{v}^\star\right\|^2\right] + c N\eta^2 \max(\sigma_{A},\sigma_{b})
%  %\left\{ \sigma_{A}^2\Verts{z^{\star}}^{2} + 3\left\{N\wedge\frac{1}{\eta\mu_g}\right\}\sigma_c^2\right\}s{N\wedge\frac{1}{\eta\mu_g}}
%   %{\eta}^2 \left(\frac{N\sigma^2_{f,2}}{\tau}\right),
% \end{align}
% for some constant $c$ independent of $N$, $\sigma_{A}$, and $\sigma_{b}$. \ps{In eq. above, by $\m v^\star$ you mean $\m z$, right? $\sigma_{A}$, and $\sigma_{b}$ have not yet been defined. Also, on the r.h.s., shouldn't the second term be $\frac{2 c \eta \max(\sigma_{A},\sigma_{b})}{\mu_g}$?}
% \end{theorem}
% %
% % \begin{wrapfigure}{r}{0.5\textwidth}
% % \begin{minipage}{0.5\textwidth}
% % \vspace{-8mm}
% % \begin{algorithm}[t]
% %   \caption{$\m{s}_N=~\pmb{\fedimvp}~(\m{s}_0, N)$} %Federated approximate inverse-Hessian product
% % \begin{algorithmic}[1]
% % \State Select $\Sc_0,\Sc_1, \ldots, \Sc_{ N'} \in \Sc$ UAR.
% %   \For{$i \in \Sc_0$ \textbf{in parallel}} 
% %   \State Compute an unbiased estimator $\hat{\m{b}}_i$ of $\m{b}_i$
% %  %\State Set $ =\hat{\m{b}}_i$
% %  \EndFor
% %  \State $ \m{v}_0 =\eta |\Sc_0|^{-1}\sum_{i\in\mathcal{S}_0} \hat{\m{b}}_{i,0}$ 
% %  \State $\m{s}_0=\m{v}_0$
% % % \State Select i.i.d.~$\Sc_1, \ldots, \Sc_{N} \in \Sc$ each drawing $B$ i.i.d.~clients with replacement% i.i.d.~Bernoulli$(p)$
% % %\State $\m{v}_0=L\m{v}$, 
% % \For{$n=1,\ldots, N$}
% % 		\For {$i \in \Sc_n$ \textbf{in parallel}} 
% % 		\State Compute an unbiased estimator $\hat{\m{A}}_i$ of $\m{A}_i$ 
% % 		 \State $\m{v}_{i,n} = \left(\m{I}-\eta \hat{\m{A}}_{i,n})\right)\m{v}_{n-1}$
% % 	   \EndFor
% % 	   \State $\m{v}_{n}=|\Sc_n|^{-1}\sum_{i\in\Sc_n} \m{v}_{i,n}$ 
% % 	   \State $\m{s}_n=\m{s}_{n-1}+\m{v}_n$
% % 		\EndFor	
% % \end{algorithmic}\label{fedihgp_algo}
% % \end{algorithm}

% %\textbf{Federated Estimator~II.} Truncating the series in \eqref{eq:neumann_expand} to $N+1$ terms, motivates an estimator $\hat{\m{z}}$ of the form
% % \begin{equation}\label{eq:nn_estimator}
% % \hat{\m{z}}:= \sum_{j=0}^N \eta \left(\m{I}-\eta \left( \sum_{i=1}^m\m{A}_i\right)\right)^j \sum_{i=1}^m\m{b}_i.
% % \end{equation} 
% % Adaptive stochastic gradient methods such as \textsc{AdaGrad} (introduced independently by \citet{duchi2011adaptive} and \citet{mcmahan2010adaptive}) have been widely used in the past few years.  AdaGrad updates the stepsize $\eta_j$ on the fly given information of all previous (noisy) gradients observed along the way.  The most common variant of AdaGrad updates an entire vector of per-coefficient stepsizes. To be concrete, for optimizing a function $F: \mathbb{R}^d \rightarrow \mathbb{R}$,  the ``coordinate'' version of AdaGrad updates $d$ scalar parameters $c_j(k), k=1,2,\ldots,d$ at the $j$ iteration --  one for each $x_j(k)$ coordinate of $x_j \in \mathbb{R}^d$ -- according to $c_{j+1}(k)^2 = c_j(k)^2 + [\nabla F(\m{x}_j, \xi_j)]_k^2$ .
% % %in the noiseless setting, and $c_{j+1}(k)^2 = c_j(k)^2 + [G_j(k)]^2$ in the noisy gradient setting.   

% % One can also consider a variant of AdaGrad which updates only a single (scalar) stepsize according to the sum of squared gradient norms observed so far.  In this work, we focus instead on the ``norm'' version of AdaGrad as a single stepsize adaptation method using the gradient norm information, which we call AdaGrad-Norm. The update in the stochastic setting is as follows: initialize a single scalar $c_0 > 0$; at the $j$th iteration, iterate
% % \begin{align}\label{eqn:adagrad}
% % x_{j+1} &\leftarrow x_j - \eta \frac{\nabla F(\m{x}_j, \xi_j)}{b_{j+1}} \quad \text{with}\quad  c_{j+1}^2= c_j ^2+ \| \nabla F(\m{x}_j, \xi_j)\|^2
% % \end{align}
% % where $\eta > 0$ is to ensure homogeneity and that the units match. It is straightforward that in expectation, $\mathbb{E} [c_k^2] = c_0^2 + \sum_{j=0}^{k-1} \mathbb{E}[ \| \nabla F(\m{x}_j, \xi_j) \|^2];$ thus, under the assumption of uniformly bounded gradient $\|\nabla F(x)\|^2 \leq \gamma^2$ and uniformly bounded variance  $\mathbb{E}_{\xi}\left[\| G(x; \xi)-\nabla F(x)\|^2\right]\leq \sigma^2$, the stepsize will decay eventually according to $\frac{1}{b_j} \geq \frac{1}{\sqrt{2(\gamma^2+\sigma^2)j}}.$  This stepsize schedule matches the schedule which leads to optimal rates of convergence for SGD in the case of convex but not necessarily smooth functions, as well as smooth but not necessarily convex functions. This observation suggests that AdaGrad-Norm should be able to achieve convergence rates for SGD, but \emph{without having to know Lipschitz smoothness parameter of $F$ and the parameter $\sigma$ a priori} to set the stepsize schedule.  
% % \begin{definition}[Adaptive Neumann Series] Let $\m{C}$ be a preconditioner matrix with full rank. Then, we have the following adaptive Neumann series:
% % \begin{align}\label{eq:precond:inverse:estimator}
% % \m{A}^{-1} \approx N \m{C}\prod\limits_{n=1}^{N'}\big(\m{I}-  \m{A}(\xi_{n}) \m{C}\big)\m{b}(\zeta).
% % \end{align}
% % A sufficient condition for convergence of the above estimator is  $\left\|\m{I}- \mb{E}\left[ \m{A}(\xi_{n}) \m{C}\right]\right\|< 1$.
% % \end{definition}

% % \begin{remark}
% %  Hence, the expansion in \eqref{eq:neumann_expand} is valid provided ${\|\m{I}-\eta \left(\sum_{i=1}^m\m{A}_i+ \alpha \m{I}\right)\|< 1}$, which holds if and only if $\frac{1}{m}\sum_{i=1}^m\m{A}_i+ \alpha \m{I}$ is positive definite and ${\eta < \|\sum_{i=1}^m\m{A}_i+ \alpha \m{I}\|^{-1}}$.
% % \end{remark}

% % Applying the Neumann series expansion \eqref{eq:neumann2} to the matrix inverse appearing in \eqref{eq:solution2}, we have 
% % \begin{equation}\label{eq:neumann_expand}
% %  \m{z} =\eta \sum_{j=0}^\infty\left(\m{I}-\eta \left(\sum_{i=1}^m\m{A}_i\right)\right)^j \sum_{i=1}^m\m{b}_i.
% % \end{equation}
% % Truncating the series in \eqref{eq:neumann_expand} to $N+1$ terms, motivates an estimator $\hat{\m{z}}$ of the form
% % \begin{equation}\label{eq:nn_estimator}
% % \hat{\m{z}}:= \sum_{j=0}^N \eta \left(\m{I}-\eta \left( \sum_{i=1}^m\m{A}_i\right)\right)^j \sum_{i=1}^m\m{b}_i.
% % \end{equation}



% Given mappings $\funco:\mathbb{R}^{d_0}\times \mathbb{R}^{d_1} \dots \times \mathbb{R}^{d_N} \mapsto \mathbb{R}^{d_0}$ and $\funcin^n:\mathbb{R}^{d_{n-1}}\times \mathbb{R}^{d_n} \mapsto \mathbb{R}^{d_n}$  for $n \in [N]$, our goal is to find the unique fixed-points $\m{x}^*,\m{z}^{1,*},\dots, \m{z}^{N,*}$ such that
% \begin{equation}\label{fedblo:prob2}
% \sum_{i=1}^m \mb{F}_i\left(\m{x}^*,\{\m{z}^{n,*}\}_{n=1}^N\right)=\sum_{i=1}^m\mb{G}^n_i\left(\m{z}^{n-1,*},\m{z}^{n,*}\right)=0.
% \end{equation}
% % \begin{subequations}\label{fedblo:prob}
% % \begin{align}
% % \end{align}
% % \end{subequations}
% % \begin{subequations}\label{fedblo:prob}
% % \begin{align}
% % \begin{array}{ll}
% % \underset{\m{x} \in \mb{R}^{{d}_1}}{\min} &
% % \begin{array}{c}
% % f(\m{x})=\frac{1}{m} \sum_{i=1}^{m} f_{i}\left(\m{x},\m{y}^*(\m{x})\right) %{\rm\sf (outer)} 
% % \end{array}\\
% % \text{subj.~to} & \begin{array}[t]{l} \m{y}^*(\m{\m{x}})
% % %=
% % \in \underset{ \m{y}\in \mb{R}^{{d}_2}}{\textnormal{argmin}}~~\frac{1}{m}\sum_{i=1}^{m} g_i\left(\m{x},\m{y}\right). % ~~~~~~~~~~~~~~~~~~~~{\rm\sf (inner)} 
% % \end{array}
% % \end{array}
% % \end{align}
% Recall that $m$ is the number of clients. Here, to model mapping heterogeneity, each client $i$ is allowed to have its own mappings $(\m{p}_i,\m{s}_i)$. Moreover, we consider a general stochastic oracle model, access to local functions $(\m{s}_i,\m{p}_i)$ is via stochastic sampling as follows:% over stochastic functions (e.g.~local client data)
% \begin{align}
% \nonumber 
% \mb{F}_i\left(\m{x},\{\m{z}^{n}\}_{n=1}^N\right) &:= \mb{E}_{\xi \sim \mc{C}_i}\left[ \mb{F}_i\left(\m{x},\{\m{z}^{n}\}_{n=1}^N\right)  + 
%  \xi\right],\\ 
%  \mb{G}^n_i\left(\m{z}^{n-1},\m{z}^{n}\right) &:= \mb{E}_{\zeta \sim \mc{D}_i}\left[ \mb{G}^n_i\left(\m{z}^{n-1},\m{z}^{n}\right)+ \zeta \right],
% \end{align}
% %\end{subequations}
% %are the loss functions of the $i^{\text{th}}$ client, 
% where $(\xi, \zeta)\sim(\mc{C}_i, \mc{D}_i)$ are sampling distributions for the $i^{\text{th}}$ client. 
% %We emphasize that for $i \neq j$, the tuples $(f_i,g_i,\mc{C}_i, \mc{D}_i)$ and $(f_j,g_j,\mc{C}_j, \mc{D}_j)$ can  be different.
